Improving the Decision-Making Process of Self-Adaptive Systems by Accounting for Tactic Volatility

When self-adaptive systems encounter changes within their surrounding environments, they enact tactics to perform necessary adaptations. For example, a self-adaptive cloud-based system may have a tactic that initiates additional computing resources when response time thresholds are surpassed, or there may be a tactic to activate a specific security measure when an intrusion is detected. In real-world environments, these tactics frequently experience tactic volatility which is variable behavior during the execution of the tactic. Unfortunately, current self-adaptive approaches do not account for tactic volatility in their decision-making processes, and merely assume that tactics do not experience volatility. This limitation creates uncertainty in the decision-making process and may adversely impact the system's ability to effectively and efficiently adapt. Additionally, many processes do not properly account for volatility that may effect the system's Service Level Agreement (SLA). This can limit the system's ability to act proactively, especially when utilizing tactics that contain latency. To address the challenge of sufficiently accounting for tactic volatility, we propose a Tactic Volatility Aware (TVA) solution. Using Multiple Regression Analysis (MRA), TVA enables self-adaptive systems to accurately estimate the cost and time required to execute tactics. TVA also utilizes Autoregressive Integrated Moving Average (ARIMA) for time series forecasting, allowing the system to proactively maintain specifications.

==> 03-problem_definition_jeff.tex <==
\section{Problem Definition}
\label{sec:proposedTechniqueThesis}
To define the key concepts and problems addressed in our work, we will use a self-adaptive web service scenario as our motivating example. 

%To define the problem addressed by our work, we will use a self-adaptive web service scenario as our motivating example. In this section, we describe what potential Service Level Agreement (SLA) requirements might look like for the system while also demonstrating the problem of not accounting for tactic volatility.

\subsection{Monitoring SLA Requirements}
\label{sec:slaTimeSeries}

First, we will define what an SLA might look like for a self-adaptive web service. One of the main requirements of this web service is that ``\textit{response time is not allowed to, or should not, surpass specific thresholds}''. Meaning, when response times surpasses some threshold, the web service is going to experience some kind of penalty as defined in the SLA~\cite{Jung:2009:CAE:1813355.1813367}. This may come in the form of overloaded servers or interruptions in loading content causing negative impacts to the user experience. For this scenario specifically, a basic SLA with requirement ($REQ$) possessing our arbitrarily defined penalties ($P$) and rewards ($RWD$) may be defined as:


\[ 
    SLA=
    \begin{cases} 
      REQ = $response time \leq$ 3 seconds \\
      P = $3$ \\
      RWD = $10$
   \end{cases}
\]
\vspace{2mm}

Real-world systems typically have more than one defined requirement. Therefore, it is imperative that the system has the ability to know \textit{what} requirements to address and \textit{when} to address them. Fortunately, this can be determined by another component of the SLA. By examining the defined reward ($RWD$) for requirements, the system is able to know the exact order in which requirements need to be addressed since ($RWD$) represents how much ``reward'' the system gains from maintaining the requirement. If the web service also had the following requirement where $capacity$ represents the maximum load for a server:

\[ 
    SLA=
    \begin{cases} 
      REQ = $server loads \leq .75*capacity$ \\
      P = $2$ \\
      RWD = $7$
   \end{cases}
\]
\vspace{2mm}

\noindent
and determined that both needed to be addressed, it would first address the response time issue, and then handle the server load issue since the reward for the former is greater than that of the latter.
%TRAVIS: interesting future work could be the selection of multiple lower reword requirements if the sum of their reward is greater than a larger reward requirement if a choice had to be made.

Knowing all of this still does not allow the web-service to properly maintain its requirements. To accomplish this, the system must become ``proactive" rather than ``reactive", by predicting when a requirement may be broken in the future and adapting to handle this change before it becomes problematic.

%TRAVIS: this was a bit redundant from the introduction and we're short on space
%In many of today's self-adaptive processes, systems adapt to surrounding changes in a ``reactive" manner. For example, if the web-service was acting in a reactive manner it would not adapt to broken requirements until they were actually broken. This inevitably would lead to the system experiencing the penalty defined for the requirement since it is now broken, possibly leading to further issues within the system. However, if we provide the web service the ability to know when a requirement may be broken in the future, the system could adapt and handle this change before it becomes an issue -- thus acting in a ``proactive'' manner.   

\subsection{Tactic Latency}

The amount of time necessary to complete an implementation of a tactic is known as \emph{tactic latency}~\cite{camara2016analyzing}. Self-adaptive systems must account for tactic latency as accurately as possible since it can have a large impact on the decisions the system makes. The selection and time to invoke appropriate tactics for an encountered scenario should depend on ensuring the tactics selected are available when needed~\cite{moreno2017adaptation}. In reality, these tactic latency times can be highly volatile due the environments the system is operating in. Thus, it is imperative that the system has a reliable, accurate way to estimate latency.

%The anticipated latency of a tactic can impact the selection of the most appropriate tactic(s) for an encountered scenario, and when the tactics are invoked to ensure that they are available when needed

Since the success of a web service heavily depends on how network traffic is managed, whether it be to regulate resource consumption or provide a fluent user experience, dealing with tactic latency plays a crucial role in maintaining viable operations. For example, when a web service experiences spikes or elongated times of increased network traffic, it can account for this in two ways: (I) Reduce the amount of content they are showing to the user at a time, or (II) adding additional servers to support the increased network traffic. For the web service, these two options would be considered the available tactics. The former has negligible latency, but the latency of the latter can be on the order of minutes. Therefore, if the service determines that more servers are needed to handle the increase in network traffic, it is imperative that it anticipates this time accurately. For example, the web service may define that adding a server only takes one minute to become available (\ie, the static approach to defining tactic latency). Due to this, it may decide that it is not worth reducing content shown to the user in the mean time. However, if the additional server suddenly takes four minutes to become available, the system has now found itself in a no-win scenario. Not only was the static assumption of latency extremely off, but the system could have already been dealing with the network traffic slightly by reducing content shown to the user. \textit{Therefore, accounting for tactic latency volatility is a paramount concern.}


\subsection{Tactic Cost}

An extremely common process in web services is the backing up of data by sending it to servers or logging it internally through their networks. Transmitting this data regularly to backup servers is crucial for some systems because it may contain user activity, account info, or person informational that would be detrimental if lost. Since the self-adaptive web service could potentially use battery power, the energy cost to perform this action will likely be a primary concern in deciding when to perform this data transfer process. Furthermore, it is likely that this will also dictate the frequency of this operation as well. Unfortunately, the cost for performing this action could be volatile due to numerous reasons. These could include include erratic hardware behavior (battery or another component not operating at optimal levels), or the file transfer taking longer than expected (packet loss, adversarial actions). Since the system's battery has a finite amount of energy, the relative cost of this transfer process increases as the battery level decreases. 

To demonstrate the deficiency of assuming tactic cost to be a static value, we will assume that the web service initially defined the backup process to have a cost ($C$) of $5$ units. However, after observing the backup process for a period of time, it was found that cost behaved quite erratically; returning cost values of $C=\{10, 2, 7, 12, 15\}$. This means that when using a static value, the system could have potentially performed the backup process while consuming the remaining amount of battery power, thus leading to an overall crash of the system. \emph{Therefore, when cost is a consideration in the decision-making process, volatility should be a first class-concern.}


==> TacticUncertainty-Papers (3)/00-abstract.tex <==
\begin{abstract}

When self-adaptive systems encounter changes within their surrounding environments, they enact \textit{tactics} to perform necessary adaptations. For example, a self-adaptive cloud-based system may have a tactic that initiates additional computing resources when response time thresholds are surpassed, or there may be a tactic to activate a specific security measure when an intrusion is detected. In real-world environments, these tactics frequently experience \textit{tactic volatility} %which is any unpredictable change that occurs within the tactic.
which is variable behavior during the execution of the tactic.

Unfortunately, current self-adaptive approaches do not account for tactic volatility in their decision-making processes, and merely assume that tactics do not experience volatility. This limitation creates uncertainty in the decision-making process and may adversely impact the system's ability to effectively and efficiently adapt. Additionally, many processes do not properly account for volatility that may effect the system's Service Level Agreement (SLA). This can limit the system's ability to act proactively, especially when utilizing tactics that contain latency.

To address the challenge of sufficiently accounting for tactic volatility, we propose a \emph{Tactic Volatility Aware} (TVA) solution. Using Multiple Regression Analysis (MRA), TVA enables self-adaptive systems to accurately estimate the cost and time required to execute tactics. TVA also utilizes \emph{Autoregressive Integrated Moving Average} (ARIMA) for time series forecasting, allowing the system to proactively maintain specifications. 

\end{abstract}

% DK 9/1:Maybe tweak these a bit?
\begin{IEEEkeywords}
Artificial Intelligence, Self-Adaptation, Machine Learning 
\end{IEEEkeywords}


==> TacticUncertainty-Papers (3)/01-introduction.tex <==
\section{Introduction}

The world is increasingly relying upon autonomous, self-adaptive systems that have the ability to function independently without human interaction. Examples of these self-adaptive systems include self-driving cars, medical devices, and many common Internet of Things (IoT) devices. Many self-adaptive processes utilize a closed-loop control mechanism that monitors the system's state and its surrounding environment. Furthermore, these mechanisms also determine if the system should be altered to perform any necessary adaptations~\cite{kephart2003vision, Brun:2009:ESS:1573856.1573860, salehie2009self, Dobson:2006:SAC:1186778.1186782}. These self-adaptive approaches typically rely upon a set of \emph{adaptation tactics} to make necessary changes~\cite{moreno2017adaptation, Schmerl2014ArchitecturebasedSC, 4221625, Huber:2014:MRA:2583044.2583093, Garlan2009}. Example tactics include the provisioning of an additional virtual machine in a web farm when the workload reaches a specific threshold, or reducing non-essential functionality on an autonomous Unmanned Aerial Vehicle (UAV) when battery levels are low.

Tactics frequently experience latency, which is the amount of time from when a tactic is invoked until its effect on the system is realized~\cite{moreno2017adaptation, Moreno:2018:FED:3208359.3149180, Moreno:2017:CMP:3105503.3105511, 7573126}. Examples of tactic latency include a cloud-based system requiring more than a minute to update certain firmware nodes~\cite{maatta2010program, anaya2014prediction}, or a cyber-physical system requiring one minute to re-activate GPS signals~\cite{liu2012energy, moreno2015proactive}. Tactics also frequently have a cost associated with them, which may be in the form of energy, monetary or other resource costs necessary for execution~\cite{Jung:2009:CAE:1813355.1813367,4220924,CostBenefitAnalysis}. Examples of tactic cost include the required energy for moving a physical component in a UAV or the monetary cost of using a remote third-party resource for computational tasks.

Both tactic latency and cost are likely to be first-class concerns in the decision-making process, as they can directly impact if and when a tactic is executed~\cite{moreno2017adaptation, Moreno:2017:CMP:3105503.3105511, 7573126}. Improperly accounting for tactic latency can lead to situations where tactics are begun too early or too late, or are not available when needed~\cite{moreno2017adaptation, Moreno:2018:FED:3208359.3149180}. Additionally, improperly accounting for tactic cost can result in the selection of a tactic that is more expensive than a tantamount, less costly alternative~\cite{CostBenefitAnalysis}. Therefore, it is imperative that self-adaptive systems properly account for both the latency and cost of tactics.

Real-world systems will frequently encounter \emph{tactic volatility}, which is any rapid or unpredictable change that exists within the attributes of a tactic. For example, both tactic latency and cost may be highly volatile depending on the system's surrounding environment. A tactic of transmitting data could take longer than expected due to network congestion, or a tactic of moving a physical component in a UAV could be more expensive due to mechanical problems.

Unfortunately, state-of-the-art decision-making processes in self-adaptive systems do not account for tactic volatility. This limitation can be highly problematic, adversely impacting the decision-making process in several ways. For example, a system may execute a tactic too late to be effective if it assumes that the tactic will always take two seconds to conduct, when in reality it has been observed to consistently take longer.

A \emph{Service Level Agreement} (SLA) helps to define system objectives such as keeping a value under a specific threshold, along with rewards and penalties for meeting defined objectives~\cite{moreno2017adaptation}. A challenge for purely reactive processes is that the system may not adhere to objectives defined in the SLA if tactics are expected to experience latency. For example, the SLA for a cloud-based self-adaptive system may define a reward for operating under a response time threshold. However, tactics such as adding servers to reduce response times will likely experience varying levels of latency. To perform optimally, the system should act proactively by beginning these tactics \emph{before} the additional resources are required so that the resources are available when needed~\cite{7573126,camara2014stochastic}. Thus, a mechanism that enables the system to accurately forecast tactic latency and cost values is highly beneficial to the self-adaptive process.

%\hl{In systems where the SLA plays a smaller role in the decision-making process, these tactic estimations can still be included in these systems to benefit their decision-making process.}\dan{added. Do you think that I said enough here, or is it confusing?}

%\hl{In some cases, the SLA will comprise only a portion of a system's decision-making process. In these situations, the tactic estimations can benefit the system by being incorporated into the specific decision-making process.}\dan{added. Do you think that I said enough here, or is it confusing?}

% In systems where the SLA plays a smaller role in the decision-making process, these tactic estimations can still be included in these systems to benefit the decision-making process.

%\hl{When the SLA comprises only a component of the decision-making process, the tactic estimations can still be included in the specific decision-making process to similarly benefit these systems as well.}\dan{added}

% What are we doing
% (Be sure to clearly describe what we are doing Give the reader a complete topical understanding of our process)
To address the limitations of current self-adaptive processes in properly accounting for tactic volatility, we propose a \emph{Tactic Volatility Aware} (TVA) solution. Through the use of a Multiple Regression Analysis (MRA) model, TVA enables the self-adaptive system to learn from previously experienced tactic volatility and make accurate estimates of how the tactic will behave in the future. TVA also includes an \emph{Autoregressive Integrated Moving Average} (ARIMA) component to enable self-adaptive systems to proactively begin adaptations according to their SLA specifications. 

To summarize, this work makes the following contributions:
\begin{enumerate}[noitemsep]

    \item \textbf{Problem Demonstration: }Using simulations, we demonstrate that accounting for tactic volatility is essential in self-adaptive systems, especially when the system is known to have unpredictable behavior.

    \item \textbf{Concept: }To the best of our knowledge, our TVA approach is the first process that accounts for tactic volatility. Existing processes merely consider tactics to have static values, whereas our TVA approach uses run time predictions of latency and cost to handle tactic volatility.

    \item \textbf{Experiments: }Our experiments demonstrate the positive impact that TVA has on the decision-making process. These experiments are conducted using real-world data, and thus provide additional confidence in our findings.

%We conducted several experiments using real-world scenarios and datasets that emulate a self-adaptive system to demonstrate the positive impact TVA has on the decision making process. These experiments are conducted using real-world data, and thus provide additional confidence in our findings. 

    \item \textbf{Tool and Dataset: }Our VolAtiLity EmulaTor (VALET) tool includes data generated from a physical system. This enables the evaluation of our TVA process and provides other researchers with a foundational dataset that they may use to support their own research. This tool and dataset are available on the project website: \ToolURL

    % DK: It might not be a bad idea to reword this a bit, make sure that people know that the data is a bit more generic

\end{enumerate}

The rest of the paper is organized as follows. Section~\ref{sec: problemdefinition} motivates our research using examples of tactic volatility. Section~\ref{sec:proposedTechniqueThesis} defines our TVA solution to effectively address tactic volatility. Section~\ref{sec: VALETTool} describes \emph{VALET}, our tactic volatility dataset. Section~\ref{sec: Evaluation} describes our systematic experimental evaluation of our proposed process. Section~\ref{sec: relatedworks} describes related works, while Section~\ref{sec: threats} describes threats and future work. Section~\ref{sec: conclusion} concludes our work.


==> TacticUncertainty-Papers (3)/02-related_work.tex <==
\section{Related Works} 
\label{sec: relatedworks}

Although our work is, to the best of our knowledge, the first known to make tactic volatility a first-class concern in the self-adaptive decision-making process, previous works have examined the impact of tactic latency in self-adaptive systems. C{\'a}mara \etal\cite{camara2014stochastic} was likely the first to consider tactic latency and examined how considering latency could be used to assist the proactive adaptation process. However, this work differs from TVA in that it does not consider any forms of tactic volatility that are likely to be encountered.


In SB-PLA, the latency of an adaptation is considered in the adaptation decision-making process~\cite{kwiatkowska2004probabilistic}. A primary benefit of SB-PLA is that systems that cannot use tactic-based adaptations can still include latency awareness in their decision-making process~\cite{moreno2017adaptation}. In addition to supporting pro-activeness and concurrent tactic execution, PLA techniques also account for latency. PLA considers the amount of time necessary for a tactic to execute, in order to avoid situations that are not achievable when time dimensions are recognized. However, like with many latency aware approaches, latency is still considered to be a static attribute. In our work, we do not consider latency to be static and provide the system with the ability to predict tactic latency at run time.

Jamshidi \etal\cite{Jamshidi:2015:SCC:2861850.2861987} presented \texttt{FQL4KE}, a self-learning fuzzy cloud controller. This enables systems to not rely upon design-time knowledge, but allows users to simply adjust weights that represent system priorities. This work found that their proposed process outperformed a previously devised technique that did not have a learning mechanism. Our work is similar in that we both utilize learning to enable the system to make better decisions. However, our work differs in that Jamshidi \etal focused on improving resource planning, and not in addressing tactic volatility as is accomplished by TVA.

%% Cost
While our work is the first to account for \emph{cost volatility}, existing research has considered cost in the self-adaptive decision-making process. Several works have included cost in their utility equations, however they consider it to be a static value and do not account for real-world volatility~\cite{Moreno:2018:FED:3208359.3149180, 7573126, moreno2017adaptation, moreno2015proactive}. Jung~\etal\cite{Jung:2009:CAE:1813355.1813367} demonstrated that ignoring cost can have a significant impact on the ability to satisfy response-time-based SLAs. This work also proposed a cost-sensitive self-adaption engine using middleware to create adaptation decisions. This work differs from ours in that it only considers cost in cloud-based controllers, while we focus on cost during the entire decision-making process.

Esfahani \etal\cite{esfahani2013learning} utilized learning to improve the self-adaptive process. A primary contribution of this work is a new process of reasoning and assessing adaptation decisions using online learning. A preliminary work by Elkhodary~\cite{7503491} proposed combining feature-orientation, learning and dynamic optimization techniques to create a new class of self-adaptive systems that would be able to modify their adaptation logic at run time. TVA differs from this work in that learning is utilized to predict tactic latency and cost at run time, while also providing away to estimate future values for requirements. 

Kinneer \etal\cite{kinneer2019information} developed a process for reusing prior planning knowledge to help the system to adapt to unexpected situations. This process considered that tactics may fail, and supports reasoning about tactic latency. While this work is helpful for assisting the overall planning process, it does not enable the system to actively learn and predict future values for tactic latency and cost like our TVA approach does.


% DK: Review these to see if any of them should be cited


%On Learning in Collective Self-adaptive Systems: State of Practice and a 3D Framework



Machine learning has been utilized to help determine the most efficient configurations for self-adaptive systems, while also performing adaptation planning. Quin \etal\cite{Quin:2019:EAL:3341527.3341529} enhanced the traditional MAPE-K feedback loop through the use of a learning model that selects subsets of adaptation options from a larger set of adaptation possibilities. This process enables the system to make more efficient analysis decisions. Jamshidi \etal\cite{Jamshidi:2019:MLM:3341527.3341534} used machine learning to discover Pareto-optimal configurations to eliminate the need to explore every configuration. This work also restricted the search space necessary to make planning tractable. These works differ from ours in that while they use machine learning to create a more efficient self-adaptive process, they do not use machine learning to address the issue of tactic volatility.

% DK: 9/13/19 Remove if space is an issue, but can add back in if we have room.

%Cheng \etal\cite{Cheng:2012:SLA:2381464.2381594} proposed a language for self-repair that includes a utility function incorporating the success rate of tactics, and thus the history of applying tactics. While similar to our work in that it incorporates prior history into its utility equation, this work does not incorporate learning mechanisms or address tactic volatility as we have.\dan{Added}

%% Dataset related works - Remove if space is an issue
The popular FIFA 98 dataset~\cite{arlitt2000workload, ita.ee.lbl.gov_Fifa_URL} is a collection of requests made to the 1998 World Cup website over an approximately four month span. This dataset is widely used in self-adaptive research and can be used to simulate when new servers would have to be activated up to handle additional web traffic or when to disable resource heavy features on a website because the traffic load is impeding the system. However, this dataset does not contain latency. Each request is a log entry that consists of information such as timestamp, size, status, and URL hit. Because this dataset does not contain any latency information, such as a request received and request fulfillment time, it cannot be used in collaboration with researching and evaluating latency-aware strategies such as our proposed TVA process.

%% Describe the exemplars
%Several existing self-adaptive systems artifacts and model problems (exemplars)~\cite{SEAMS_Exemplars_URL} contain artifacts which act on real-world data and/or can be accessed remotely for experimentation. However, no known exemplars contain datasets that contain significant amounts of cost or latency volatility created from a real-world environment.





%D'Angelo \etal\cite{8787033} % Not really related at all


% DK: If space is an option, maybe add a section/portion on ARIMA or another one of the utilized learning processes

==> TacticUncertainty-Papers (3)/03-problem_definition_dan.tex <==
\section{Problem Definition} 
\label{sec: problemdefinition}

\emph{Tactic latency volatility} and \emph{tactic cost volatility} are the primary motivators for addressing a system's SLA with proactive processes. If a system is purely reactive and does not properly anticipate future system changes in regards to the specifications defined in the SLA, it will be limited by its inability to provide support for proactive tactic implementation. %\hl{We further motivate this problem by using an example derived from Moreno} \etal\cite{moreno2017adaptation}.\dan{remove this?}

\subsection{Tactic Cost Volatility}

Examples of tactic cost vary widely and are largely domain specific, however tactic cost is frequently a primary concern in the decision-making process~\cite{CostBenefitAnalysis}. Possible examples of tactic cost include the energy necessary to move a mechanical component in a physical device, the monetary cost to utilize a resource, or the number of computations necessary to perform a tactic. Estimating tactic cost will likely be a first-class concern for the system, especially if there are defined cost thresholds, resource limitations, or if the system merely has the goal of attaining maximum utility at the lowest cost~\cite{moreno2017adaptation}. Unfortunately, despite the cost volatility that many real-world systems are likely to encounter, existing self-adaptive processes that account for cost consider it to be a static value that will encounter no volatility~\cite{Moreno:2018:FED:3208359.3149180, 7573126, moreno2015proactive}. Accounting for tactic cost volatility is imperative for several reasons:

\begin{enumerate}[noitemsep, nosep]

    \item \descStep{Cost may be a primary consideration when selecting between multiple tactic options}{When the system has multiple tactic options that it may choose from, the cost of the tactic may be a determining factor when selecting between multiple, otherwise tantamount options.}
    
    %the SLA it will help to define the expected reward, penalties and cost. The system will then use this input to make its tactic decisions. Therefore, when considering between multiple tactic options, it is important to have an accurate cost estimate to ensure that the most optimal tactic option(s) are selected by the system.
    
    \item \descStep{Determine if the cost exceeds reward}{In selecting which tactic(s) to execute, the system will frequently calculate the expected reward and cost for performing the tactic. If the cost exceeds the reward, then it may not be optimal for the system to execute the tactic.}
    %Therefore it is imperative for the system to have an accurate cost estimation for performing the tactic.}
    
    \item \descStep{The estimated cost may impact the system's ability to execute concurrent or subsequent tactics}{The system may possess a finite amount of a resource, with one example of being battery power. Assume that a system has 10 units of battery power remaining. Processes that consider cost to be a static value may define the energy usage of tactic $a=4$, and for tactic $b=5$. Therefore the system will assume that it has the ability to execute both tactics concurrently or sequentially. However if the actual energy usage of each tactic is $a=6$ and $b=7$, in reality the system will not have the ability to fulfill the amount of energy necessary for the execution of both tactics either concurrently or sequentially.}

\end{enumerate}


\subsection{Tactic Latency Volatility}

The amount of time required to implement a tactic is known as \emph{tactic latency}~\cite{camara2016analyzing}, which in real-world systems, can be highly volatile. %Some tactics such as updating firmware nodes in cloud-based systems may take more than a minute to update~\cite{maatta2010program, anaya2014prediction} and in a cyber-physical system, the tactic of re-activating the GPS may take over a minute~\cite{liu2012energy, moreno2015proactive}. 
%Some tactics such as retrieving a file from a remote location can take anywhere from several milliseconds to several days.
For example, the precise amount of time a system needs to transmit a file across a network may fluctuate due to varying amounts of network traffic. Previous works have shown that latency aware self-adaptive processes offer several advantages over traditional, non-aware techniques~\cite{camara2014stochastic, moreno2017adaptation, Moreno:2018:FED:3208359.3149180}. However many state-of-the-art self-adaptive processes still consider tactic latency to be a predetermined and static value. Systems lack the capability to learn to adaptively accommodate for variability in tactic latency. Due to its large impact on the decisions that a system should make, accounting for tactic latency volatility is imperative for several reasons:

\begin{enumerate}[noitemsep,nosep]
    \item \descStep{Knowing when to begin the execution of a tactic}{A priority for many self-adaptive systems is to ensure that tactics are ready when needed. Therefore, if a tactic has expected latency, then the system will need to proactively begin its execution so that it is available when needed. However, implementing a tactic proactively will typically have additional costs involved, so proactive adaptation must be done with consideration to available resources.}
    
    %cost is a consideration the system will not want to begin the execution of the tactic too soon so that it will not incur unnecessary costs.}
    
    %Therefore, properly accounting for tactic latency volatility is imperative for a robust system, one that is able to accurately determine when a tactic should be invoked to ensure that it is completed when needed.}


% Page 3,  “2) determine when to augment a slow tactic with a faster tactic”,  this paragraph is hard to follow. It is unclear why we need to augment a slot tactic with a faster one. And I don’t think this point is even addressed in later sections.


% There may be times when a system will need to augment a slower tactic with a faster tactic. For example, one tactic may take longer to implement but may be more beneficial than a faster tactic option. A real world example of this could be.....

% Accurate tactic latency knowledge is imperative for determining when to augment a slow tactic with a faster tactic. There may be instances when the system decides to utilize a faster, less effective tactic to augment a slower, but more effective tactic~\cite{moreno2015proactive, moreno2017adaptation}.  


% --> Make sure to address this point in later sections - DK: I am not really sure how we could do this.

    \item \descStep{Determine when to augment a slow tactic with a faster tactic}{Accurate tactic latency knowledge is imperative for determining when to augment a slow tactic with a faster tactic. There may be instances when the system decides to utilize a faster, less effective tactic to augment a slower, but more effective tactic~\cite{moreno2015proactive, moreno2017adaptation}. For example, in a self-adaptive system some given tactic $a$ may have higher latency while producing a higher benefit than that of a faster tactic option $b$. The system may decide to implement both tactic options, knowing that the system could potentially realize the benefits of tactic $b$ while it is waiting for tactic $a$. When deciding to augment a slower tactic with a faster one, accounting for tactic latency volatility is essential to determine which tactic(s) should be used to augment a slower tactic.}
    
    %required to determine: (I) When to augment a slow tactic with a faster one, and (II) Which tactic(s) should be used to augment a slower tactic. \dan{All: Please review}} 

%    \item \descStep{Determine when to augment a slow tactic with a faster tactic}{Accurate tactic latency knowledge is imperative for determining when to augment a slow tactic with a faster tactic. There may be instances when the system decides to utilize a faster, less effective tactic to augment a slower, but more effective tactic~\cite{moreno2015proactive, moreno2017adaptation}. Accounting for tactic latency volatility is required to decide: (I) When to augment a slow tactic with a faster one, and (II) Which tactic(s) should be used to augment a slower tactic.} % Not accounting for tactic latency volatility can lead to scenarios where the system 

    \item \descStep{Ensuring the selection of the most appropriate tactic}{When selecting between multiple tactic options, ignoring tactic latency can be problematic. Consider a scenario where the system is deciding whether to use tactic $a$ or tactic $b$. If tactic $b$ is only slightly better than tactic $a$ in terms of instantaneous utility improvement, then the decision-making process would favor tactic $b$. However, if tactic $a$ is faster than tactic $b$, then tactic $a$ would start to accrue utility faster. This means that tactic $a$ may be the most optimal selection~\cite{moreno2015proactive}.}% Due to the importance of tactic latency in this scenario, tactic latency \emph{volatility} will be an equally important consideration, since varying tactic latency will impact the selection of the most appropriate tactic.}

%    \item \descStep{}{}
%    \item \descStep{}{}
\end{enumerate}





% Proactive SLA Forecasting

%\subsection{Forecasting SLA Specifications} % Change this title

%The \emph{Service Level Agreement} (SLA) helps to define how utility is calculated in self-adaptive processes. 

%The SLA may define specific system specifications, with defined rewards and penalties~\cite{jung2009cost}. For example, the SLA may define a maximum response time threshold for server responses in a self-adaptive hosting environment or another similar specification. If a system is purely reactive, and does not properly anticipate future system changes in regards to the specifications defined in the SLA, it will be limited by its inability to provide support for proactive tactic implementation. 


%Many tactics have latency, so anticipating future system needs will enable the system to proactively adapt before the tactic is actually needed.



%for several reasons:\dan{This could be more convincing}

%While SLAs are common in self-adaptive systems, many self-adaptive systems are only capable of anticipating when current actions are going to violate SLA specifications......\dan{add to this}


% Give a specific example of the problem that we will be solving here
%A system that is purely reactive, and does not `Lookahead' to future ?states? in regards to how it will perform in respect to its SLA will be limited for several reasons:


%\begin{enumerate}[noitemsep]

%    \item \descStep{Provide support for proactive tactic implementation}{Since many tactics have latency, anticipating future system needs will enable the system to proactively adapt before the tactic is actually needed.}
%    \item \descStep{Support specifications not being violated in the first place}{In a purely reactive system, the system may encounter a penalty/lost reward before the system has a chance to adapt. A proactive approach would enable the system to never encounter this problem in the first place. \dan{not sure if this is true. - It might not be a bad idea to remove this one}}

% what can we take from PLA - What are the reasons that they give?


%    \item \descStep{Provide support for proactive tactic implementation}{If tactic has latency and takes time to implement, predicting when SLA xviolationsx will occur will enable the system to start tactics before they are needed. This will better enable the tactics to be ready when necessary} % ? How does this tie back into the tactic volatility thing?

%    \item \descStep{Add more}{\dan{Jeff: Are there any others?}}

%\end{enumerate}




% Even with no tactic latency, you will still experience the penalty/lose the reward while you are being hit with it

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Be sure to define SLA someplace in the introduction as well
%   Might also not be a bad idea to limit this section and focus more on the BRR stuff
% Might improve this by making it more about 

% Give a basic definition of things
%The \emph{Service Level Agreement} (SLA) helps to define how utility is calculated in the self-adaptive system \todo{cite}. The SLA may define specific system objectives, with defined rewards for meeting specific objectives, and defined penalties for not meeting these objectives~\cite{jung2009cost}. The specific attributes of the SLA will be defined by the engineers and will be highly domain specific. For example, the SLA may define a maximum response time threshold for a self-adaptive hosting environment, or XXXXX.  %DK: Add citations - take the examples from specific papers

% Define the problem that we are solving. What is the need for future work in this area

%While SLAs are common in self-adaptive systems, most self-adaptive systems are only capable of anticipating when current actions are going to violate SLA requirements. A process that would enable the 


%Most systems have no way to act proactively in ensuring that the SLA is adhered to in order to ensure that the system performs as optimally as possible.% DK: Removed since this is a strong statement, maybe other works are doing this


%While SLAs are common in self-adaptive systems, most self-adaptive systems are only capable of anticipating when current actions are going to violate SLA requirements. To help ensure that future system states do not violate objectives defined in the SLA, it is important to provide the system with \emph{proactive} predictive abilities to identify when SLA objectives will likely be violated in the future. This would provide the system with the ability to make appropriate adjustments in anticipation of violations. Acting proactively is important since many systems will not be able to make the appropriate adaptation adjustments instantaneously, and will require some time\todo{cite}. While existing works provide systems to act proactively\todo{cite}, none focus on supporting the system's ability to act proactively in regards to the SLA. %weak


%they do not enable the system to act proactively and anticipating when the system's future 

%not looking ahead to predict where the system will be in a future state, providing the system with the ability to act proactively before SLA requirements are xBrokenx




% Briefly mention how PLA etc..... attempt to do this, but fall short
%   Will need to add to this in the related works section



%   MDP
%   PLA
%   Other forecasting techniques


% Make predictions of future values based on requirements defined in the threshold. Since the items defined in the SLA can be highly domain specific, we will use the example of a threshold ($T$), since it is very commonly used in self-adaptive research~\cite{XXAdd in citationsXX}

% Maybe provide a specific example to provide a bit more context


% Describe how XXXXX are defined in the SLA
% Threshold is an example

% Look at QoS as well



\subsection{Motivating Example} 
\label{sec: motivatingexample}

As a motivating example we will use a cloud-based self-adaptive system, based on a similar scenario defined by Moreno \etal\cite{moreno2017adaptation}. This example represents a multi-tier web application that is compromised a web server and database tier. The webserver(s) process a client's request and then access information stored in the database tier. To efficiently provide content while encountering variable workloads, the system can either add/remove servers from the pool or reduce optional content using the `dimmer' feature. This system has has a goal of maximizing utility while minimizing cost.%\dan{updated previous sentences} 

The SLA defines the target response time ($T$) and how utility ($U$) is calculated. The system incurs penalties if the target response time is not met and accrues rewards for meeting the target average response time against the measurement interval. %In this scenario, the cost is directly proportional to the number of servers used. 
The average response rate is $a$, the average response time is $r$, the maximum request is $k$ and the length of each interval is defined as $\tau$. Provided content is reduced as necessary using a dimmer value ($d$). Optional content has reward of ($R_O$), and produces a higher reward than mandatory content ($R_M$). We will slightly modify the equation to incorporate cost ($C$), which could be the monetary or energy cost:

\begin{equation} \label{eq: motivatingExample}
	U = \left\{ \begin{array}{rl}
 	(\tau a (dR_O+(1-d)R_M)/C~~~~r\leq T \\ 
  	(\tau \min (0,a-k)R_O)/C~~~~r> T 
       \end{array} \right.
\end{equation}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%As a motivating example, we will utilize a scenario derived from Moreno \etal\cite{moreno2015proactive}. In this scenario, the goal of this example cloud-based self-adaptive system is to provide user content while maximizing the difference between revenue and cost, with server cost being represented by $C$. The system must provide requested content under a response threshold time of $T$, with responses above this time returning no revenue. The system provides mandatory ($M$) and optional ($O$) content with their respective revenue being $R_0 > R_M > 0$. The number of servers at time $t$ is represented by $s(t)$. $x_O$ and $x_M$ are the number of responses with a time~$< T$ for each kind of response. There must be one server running at all times, and therefore the first server is not included in the cost. If the system runs for duration $L$, the total utility (\ie the difference between revenue and cost) is represented by Equation~\eqref{eq: LatencyExample}. 

% Cost per server unit time

%\begin{equation} \label{eq: LatencyExample}
%U = R{_o}x_o + R{_M}x_M -C \int^L_0 (s(t)-1) \mathop{}\!\mathrm{d}t
%\end{equation}


This system can account for increases in user traffic using two different tactics: (I) reducing the proportion of responses that include the optional content (dimmer), and (II) adding a new server. While reducing optional content will have negligible latency, adding a new server can take several minutes.%~\cite{moreno2017adaptation}. %? cite

\vspace{0mm} \noindent \textbf{Tactic Latency Volatility} If the system anticipates that the response threshold will be surpassed in the immediate future, then the system could proactively start the tactic of adding a server to keep the response time under the defined threshold. Overestimating latency could result in scenarios where the system unnecessarily incurs additional cost, as servers would be `active' longer than necessary. Additionally, if the system determines that it is likely to surpass the defined response time threshold before a new server can be added, then the most appropriate system action may be to use the faster tactic that reduces the amount of optional content while it waits for a new server to be added. Improper tactic latency predictions can lead to situations where the system executes the tactic too soon or too late, or even selects the improper tactic for the encountered scenario. \emph{Accounting for tactic latency volatility is a paramount concern, especially when utilizing a proactive adaptation approach, or when utilizing complementary tactics.} % DK: I don't love the takeaway messages in each of these examples

\vspace{0mm} \noindent \textbf{Tactic Cost Volatility} In the provided scenario, it is important to account for cost volatility, especially since not accounting for cost volatility could lead to inaccurate utility calculations. In the event that cost is defined to be higher than what the system is actually encountering in the real-world, then this may lead to scenarios where optional ($O$) content is shown too infrequently. Conversely, if the cost is defined lower than what is being encountered in the real-world, then could lead to scenarios where optional ($O$) content is shown too frequently. \emph{A volatility aware solution that enables the system to more accurately predict cost would enable the system to make decisions that lead to more optimal outcomes.}

%The anticipated cost of a tactic can have a profound impact on the decision-making process of the system. In the example provided by Moreno \etal\cite{moreno2015proactive}, cost is considered to be a static, predefined value. However, in many real-world systems cost may be a highly volatile value. 

% Optional content is shown less frequently to keep costs down


% Will lead to inaccurate  utility calculations

% Cost is a significant decision on the selected tactic.

%a volatile cost value should be accounted for since it would impact the decision making 


% Cost is not a tactic value now -- How to fit in:
%   Assume that the cost of adding/removing a tactic has a monetary/energy etc value (word eloquently)


\vspace{0mm} \noindent \textbf{Reactive Specifications Monitoring} If the motivating example was a purely responsive system and did not employ any proactive functionality, it will only determine if the defined response threshold ($T$) is being surpassed at the current moment. This can be problematic since the tactic of adding additional resources to reduce response time in our example has latency, so the system will need to begin adapting \emph{before} the tactic is actually needed to be complete. Otherwise, the system will incur penalties or not realize rewards while it waits for the tactic to become available. \emph{A process that enables the system to better anticipate how it was going to act in accordance with the SLA would help the system to perform more optimally in dynamic environments.}


==> TacticUncertainty-Papers (3)/03-problem_definition_jeff.tex <==
\section{Problem Definition}
\label{sec:proposedTechniqueThesis}
To define the key concepts and problems addressed in our work, we will use a self-adaptive web service scenario as our motivating example. 

%To define the problem addressed by our work, we will use a self-adaptive web service scenario as our motivating example. In this section, we describe what potential Service Level Agreement (SLA) requirements might look like for the system while also demonstrating the problem of not accounting for tactic volatility.

\subsection{Monitoring SLA Requirements}
\label{sec:slaTimeSeries}

First, we will define what an SLA might look like for a self-adaptive web service. One of the main requirements of this web service is that ``\textit{response time is not allowed to, or should not, surpass specific thresholds}''. Meaning, when response times surpasses some threshold, the web service is going to experience some kind of penalty as defined in the SLA~\cite{Jung:2009:CAE:1813355.1813367}. This may come in the form of overloaded servers or interruptions in loading content causing negative impacts to the user experience. For this scenario specifically, a basic SLA with requirement ($REQ$) possessing our arbitrarily defined penalties ($P$) and rewards ($RWD$) may be defined as:


\[ 
    SLA=
    \begin{cases} 
      REQ = $response time \leq$ 3 seconds \\
      P = $3$ \\
      RWD = $10$
   \end{cases}
\]
\vspace{2mm}

Real-world systems typically have more than one defined requirement. Therefore, it is imperative that the system has the ability to know \textit{what} requirements to address and \textit{when} to address them. Fortunately, this can be determined by another component of the SLA. By examining the defined reward ($RWD$) for requirements, the system is able to know the exact order in which requirements need to be addressed since ($RWD$) represents how much ``reward'' the system gains from maintaining the requirement. If the web service also had the following requirement where $capacity$ represents the maximum load for a server:

\[ 
    SLA=
    \begin{cases} 
      REQ = $server loads \leq .75*capacity$ \\
      P = $2$ \\
      RWD = $7$
   \end{cases}
\]
\vspace{2mm}

\noindent
and determined that both needed to be addressed, it would first address the response time issue, and then handle the server load issue since the reward for the former is greater than that of the latter.
%TRAVIS: interesting future work could be the selection of multiple lower reword requirements if the sum of their reward is greater than a larger reward requirement if a choice had to be made.

Knowing all of this still does not allow the web-service to properly maintain its requirements. To accomplish this, the system must become ``proactive" rather than ``reactive", by predicting when a requirement may be broken in the future and adapting to handle this change before it becomes problematic.

%TRAVIS: this was a bit redundant from the introduction and we're short on space
%In many of today's self-adaptive processes, systems adapt to surrounding changes in a ``reactive" manner. For example, if the web-service was acting in a reactive manner it would not adapt to broken requirements until they were actually broken. This inevitably would lead to the system experiencing the penalty defined for the requirement since it is now broken, possibly leading to further issues within the system. However, if we provide the web service the ability to know when a requirement may be broken in the future, the system could adapt and handle this change before it becomes an issue -- thus acting in a ``proactive'' manner.   

\subsection{Tactic Latency}

The amount of time necessary to complete an implementation of a tactic is known as \emph{tactic latency}~\cite{camara2016analyzing}. Self-adaptive systems must account for tactic latency as accurately as possible since it can have a large impact on the decisions the system makes. The selection and time to invoke appropriate tactics for an encountered scenario should depend on ensuring the tactics selected are available when needed~\cite{moreno2017adaptation}. In reality, these tactic latency times can be highly volatile due the environments the system is operating in. Thus, it is imperative that the system has a reliable, accurate way to estimate latency.

%The anticipated latency of a tactic can impact the selection of the most appropriate tactic(s) for an encountered scenario, and when the tactics are invoked to ensure that they are available when needed

Since the success of a web service heavily depends on how network traffic is managed, whether it be to regulate resource consumption or provide a fluent user experience, dealing with tactic latency plays a crucial role in maintaining viable operations. For example, when a web service experiences spikes or elongated times of increased network traffic, it can account for this in two ways: (I) Reduce the amount of content they are showing to the user at a time, or (II) adding additional servers to support the increased network traffic. For the web service, these two options would be considered the available tactics. The former has negligible latency, but the latency of the latter can be on the order of minutes. Therefore, if the service determines that more servers are needed to handle the increase in network traffic, it is imperative that it anticipates this time accurately. For example, the web service may define that adding a server only takes one minute to become available (\ie, the static approach to defining tactic latency). Due to this, it may decide that it is not worth reducing content shown to the user in the mean time. However, if the additional server suddenly takes four minutes to become available, the system has now found itself in a no-win scenario. Not only was the static assumption of latency extremely off, but the system could have already been dealing with the network traffic slightly by reducing content shown to the user. \textit{Therefore, accounting for tactic latency volatility is a paramount concern.}


\subsection{Tactic Cost}

An extremely common process in web services is the backing up of data by sending it to servers or logging it internally through their networks. Transmitting this data regularly to backup servers is crucial for some systems because it may contain user activity, account info, or person informational that would be detrimental if lost. Since the self-adaptive web service could potentially use battery power, the energy cost to perform this action will likely be a primary concern in deciding when to perform this data transfer process. Furthermore, it is likely that this will also dictate the frequency of this operation as well. Unfortunately, the cost for performing this action could be volatile due to numerous reasons. These could include include erratic hardware behavior (battery or another component not operating at optimal levels), or the file transfer taking longer than expected (packet loss, adversarial actions). Since the system's battery has a finite amount of energy, the relative cost of this transfer process increases as the battery level decreases. 

To demonstrate the deficiency of assuming tactic cost to be a static value, we will assume that the web service initially defined the backup process to have a cost ($C$) of $5$ units. However, after observing the backup process for a period of time, it was found that cost behaved quite erratically; returning cost values of $C=\{10, 2, 7, 12, 15\}$. This means that when using a static value, the system could have potentially performed the backup process while consuming the remaining amount of battery power, thus leading to an overall crash of the system. \emph{Therefore, when cost is a consideration in the decision-making process, volatility should be a first class-concern.}


==> TacticUncertainty-Papers (3)/04-proposed_process.tex <==
\section{Proposed TVA Process}
\label{sec:proposedTechniqueThesis}

% General overview of the process

Our TVA process consists of the following two phases: (I) Time-series forecasting with \emph{Autoregressive Integrated Moving Average} (ARIMA) and (II) Run-time model generation using Multiple Regression Analysis (MRA); where ARIMA predicts if system specifications in the SLA may be broken in the future and MRA creates run-time models for predicting tactic latency and cost.

\subsection{Autoregressive Integrated Moving Average}
The first component of the TVA process is ARIMA, which is a commonly used approach for the prediction of time series data. ARIMA is a generalization of the ARMA (autoregressive moving average) model, which accounts for non-stationary data using differencing. A full ARIMA treatment requires the following notation, \emph{ARIMA(p, d, q)}, where $p$ represents the number of lag observations included in the model, $d$ represents the degree of differencing, and $q$ represents the size, or \emph{order} of the moving average window.

%TRAVIS: maybe put this in future work
%Another ARIMA-like model that was potentially appropriate for our work was seasonal-ARIMA (SARIMA). SARIMA applies all the same techniques that ARIMA does, but is more robust when dealing with seasonal time series data. However, upon examination of the time series data collected for this work, we did not find any seasonality within the data. 

This work uses a Box-Jenkins approach to find the best fit of a ARIMA model for predicting future time series values. This involves applying the following three steps:
%There are multiple ways in which an ARIMA model can be applied. In this work, we used the Box-Jenkins approach to find the best fit of a time series model for predicting future values. To properly apply this approach, we must apply the following three components/steps of Box-Jenkins:

%\jeff{I will shorten this box jenkins stuff a lot}

\begin{enumerate}

\item \textbf{\textit{Identification: }}The first step is to determine the order of the ARIMA model, by utilizing \textit{differencing} to transform the potentially non-stationary data to stationary data. Mathematically, differences are shown as $y_{t}'=y_{t} - y_{t-1}$, where $y_t$ represents the current observation and $y_{t-1}$ represents the immediate-prior observation. Differencing allows the model to remove any changes in the levels of time series data, thus eliminating trend and seasonality. In some cases, differencing may need to be applied a second time to obtain stationary data. This second order differencing includes subtracting another term $y_t''=y_{t-1} - y_{t-2}$ to the ARIMA model. Our work used a differencing order of $d=1$, as there was a small amount of non-stationary time series data. Following this, classic autocorrelation and partial autocorrelation plots were used to determine the order of the autoregressive and moving average terms, which resulted in $p=1$ $q=0$, respectively.

%Once we transformed the non-stationary data to stationary data, the next step was to identify the order of our autoregressive and moving average terms (i.e. $p$ and $q$). We used the classic autocorrelation and partial autocorrelation plots to do this and ended up with a $p$ order of $1$ and a $q$ order of $0$.



%One of the main reasons ARIMA is more appropriate for our work than ARMA is that ARMA has a strict assumption that the time series data will always be stationary -- therefore the model is incapable of ``identifying" any non-stationary data. When non-stationary data exists, we must transform it to be stationary. This is done through a method called \textit{differencing}, which examines the difference between consecutive observations. Mathematically, this is shown as $y_{t}'=y_{t} - y_{t-1}$, where $y_t$ represents the current observation and $y_{t-1}$ represents the immediate-prior observation. Differencing allows the model to remove any changes in the levels of time series data, thus eliminating trend and seasonality. For some cases, it is possible that differencing needs to be applied a second time in order to obtain stationary data. If we find this to be true, we refer to this as \textit{second order differencing}.


\item \textbf{\textit{Estimation:} }In order to estimate parameters for the Box-Jenkins models, we must apply a solution that can numerically approximate nonlinear equations. As the goal was to minimize a loss or error term, we used the \textit{maximum likelihood estimation} (MLE) method over a nonlinear least squares estimation to determine the model's optimal parameters.

%Like the correlation plots, there are many ways to do this whether it be a nonlinear least squares estimation or a maximum likelihood estimation. However, the goal here is to minimize a loss or error term, therefore allowing any predictions that are made to be as accurate as possible. With this reasoning, our approach uses the preferred \textit{maximum likelihood estimate} (MLE) method for estimating the models parameters. 

\item \textbf{\textit{Model Checking: }}The final step in applying a full treatment of the Box-Jenkins approach is to perform model checking. Since we have the ability to modify orders in the ARIMA model ($p$ and $q$) it is important that we optimize these parameters. In general, optimization should examine: I) if the model is overfit and II) residual errors. %\jeff{made a small tweak but it's fine how it is. There are always residual errors in models because these 'errors' are the differences between prediction and actual observed values. So there's never an 'if there are' situation} 
The former is crucial because it effects how generalizable our model is to other time series data, while the latter deals with how well the model performed in terms of predictions. After examining multiple ARIMA models by fine-tuning the three main parameters $p$, $d$ and $q$, the final ARIMA model for our work was $ARIMA(1,1,0)$. With this notation, our model is known as a \textit{differenced first-order autoregressive model}.


%In an ideal model, residuals would resemble what is known as ``white noise" or more commonly, a Gaussian Distribution. This means that the average of all the residuals is zero and that the distribution shape of the variances is symmetrical. 

%\travis{You're talking about what shoudl be done and not what you did.  Did you model check? waht were the results of that? What was the final ARIMA model?}

\end{enumerate}

\subsection{Multiple Regression Analysis}
The second component of our TVA approach deals with run time predictions of tactic latency and cost. As discussed previously, current self-adaptive processes consider these values to be static attributes. In real-world scenarios, this is an unlikely phenomena because certain events have different outcomes depending on the surrounding environment. %For example, a self-driving car may need to determine how many feet it takes to stop from 60 mph, which will vary dramatically when the road is wet compared to when it is dry. Therefore, the self-driving car must have a way to model its surrounding environment (the weather, road conditions) so it can accurately plan for how long it will take to stop. 
For example, a UAV may need to determine the time it will take to transmit a critical file to its base station. This latency could drastically vary depending on the distance of the UAV to the base station, weather conditions and even component functionality. Therefore, the UAV must have a method of modeling its surrounding environment so it can accurately anticipate the length of time required to transmit the file.

In our work we applied this same ideology to predicting tactic latency and cost. There are many different types of regression models, and even machine-learning models that could be used to accomplish this. Initially, we examined a machine-learning approach called Bayesian Ridge Regression (BRR) which through a Bayesian process allows the model to train itself over time as more data becomes available. However, we found that the required feature space for BRR was too large and that the data we collected could not support it. Therefore, our TVA approach uses Multiple Regression Analysis (MRA) to support run time predictions of tactic latency and cost. Consider a classic regression model:

\begin{equation}
	%y = \beta + \beta_1x
    y(x,w) = w_0 + \sum_{j=1}^{M-1} w_j x^j=w'x
\end{equation}

\noindent
where $x=(x^1,...,x^M)'$ with $x^0=1$ and $x^j$ being the $j$-th observation of the independent variable $x$. Given a set of $N$ training variables $(x_1,...,x_N)$ along with the observed responses $(t_1,...,t_N)$, we can solve for the best possible weights of this model through minimizing the error function:

\begin{equation}
E(w) = \frac{1}{2}\sum_{n=1}^{N}\{y(x_n,w)-t_n\}^2
\label{eq:mini}
\end{equation}

\noindent
$E(w)$ is a quadratic function of $w$ (the observation weight), which can be conveniently minimized, leading to:

\begin{equation}
	w^* = (X'X)^{-1}X't
\label{eq:weights}
\end{equation}

\noindent
where $X$ is the design matrix whose rows correspond to the observation vectors of the variables and $t=(t_1,...,t_N)'$ denotes the observed response values of $N$ variables. After minimizing Equation \ref{eq:mini}, we now have the estimated weights $w^*$ in Equation \ref{eq:weights}, which can be used by our regression model to predict tactic latency and cost.

It is important to note that regression analysis estimates the conditional expectation of the dependent variable, that is, the average value of the dependent variable when the predictor variables are fixed. Other related methods such as Necessary Condition Analysis (NCA) could be used to estimate the maximum value of the dependent variable, however, we decided that this was out of scope for our approach since estimating maximum values would be considered the \textit{worst-case scenario} for the tactic.



% Develop better name for this
%\subsection{Time Series Forecasting for Maintaining SLA Defined Specifications}

% Maybe keep this shorter

% ? DK: Also include a motivating example?
%TVA utilizes ARIMA to perform time-series forecasting for helping the system to maintain SLA defined specifications. This provides the system with the benefit of being able to act more proactively to adapt to anticipated penalties as defined by the SLA. This ARIMA-based process begins by collecting relevant specifications as defined by the SLA. Next it......\dan{Jeff: Help with this part}


%This predicted specification may then be included into any predictive functionality, such as PLA~\cite{moreno2017adaptation}, to help the system to make more appropriate, proactive decisions.

%\dan{Jeff: Add 1-2 sentences about why this process will be useful compared with PLA/existing techniques}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%TVA provides self-adaptive systems with the ability to perform a lightweight, time-series forecasting 

%TVA's forecasting component is comprised of several primary steps to enable self-adaptive systems to anticipate requirements changes, enabling the system to proactively react to predicted SLA xxxxxx.   

%\begin{enumerate}[noitemsep]
%    \item \descStep{Collect xAttributesx defined in the SLA}{TVA first records the defined penalties and rewards from the SLA. For example, using the scenario in Section~\ref{sec: motivatingexample}, TVA would record the definitions for the rewards for the optional and mandatory content ($R_O$, $R_M$), along with the defined threshold ($T$).}
%    \item \descStep{Use ARIMA to predict future states for SLA xAttributesx}{}
    
    
    % T is based off the response time. Predict future states of the response time. Determine how they will impact future states of the utility equation. Inform the system, so it may decide to act more proactively.
    
    % System will predict what the Response time will be in future states. If the R is above the defined T, then the system will determine what the most appropriate action will be. Based on cost and the other items defined in the SLA, along with expected latency and cost, it will determine which (if any) adaptation decisions are necessary. 
    
    
    % 
    
    
    % static attributes such as Rm RO will be ignored since there is nothing to predict ?
    
    
%    \item \descStep{}{}
%    \item \descStep{}{}

%\end{enumerate}


%1) Collect all of the `requirements' defined in the SLA - For example, if the system defines that the response threshold should not be above T. 
%2) Use (MM) time series forecasting to determine what the system anticipates the response time to be in the X future.
%3) If the system anticipates that the defined threshold in the SLA is going to be violated, the system will take appropriate actions (domain specific)

% What phase of MAPE-K will with this integreate into?
%   Is it even important to say

%\dan{We will need to add more specifics to this. I feel like we are a bit vague over precisely how everything comes together. This needs to be really solid}
%\dan{JEFF: Check this section}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Make this very technical
% How does this tie into MAPE-K. How will this integrate into everything. Provide the reader confidence that we understand what we are doing here


% What are MDPs





%%%%% Not sure where to move everything below

%Moreno \etal\cite{7573126} presented an approach that virtually eliminated the run-time overhead of constructing MDPs mostly offline. Through the use of formal methods, this approach exhaustively considers numerous possible system states and the combination of tactics, including the concurrent execution of tactics.

% Create a short version of this for the introduction

%Our work differs, and compliments these approaches in that: (I) We focus on accounting for the volatility of the tactic, which could be implemented into existing approaches to strengthen them (II) \hl{Through time-series forecasting, we offer a relatively lightweight prediction mechanism that can be individually implemented into the self-adaptive control loop (XX \dan{explain how later if true}), or used to enhance processes such as PLA by }\dan{Jeff: Check this - A lot of this is BS we will need to clean up} %


% Incorporate into MAPE-K



% Mention the specific improvements that our process will offer compared to MDP etc..
%   run-time overhead
%   MDP depends on the stochastic behavior of the environment, which can only be estimated at run-time and has a short horizon (top of page 2 - Efficient Decision-Making under Uncertainty)
% Constructing and MDP has a high-overhead

% This approach considers 


\vspace{1mm} \noindent \textbf{TVA Workflow}

TVA combines an ARIMA time series model with an MRA model to improve the self-adaptive process. In doing this, the system is able to properly maintain its defined specifications while also accounting for tactic volatility, leading to better adaptations and better overall performance. As shown in the pseudo code in Algorithm~\ref{alg:TVAWorkFlow}, the workflow of TVA is reasonably straightforward. The top level definitions under $procedure$ represent the specifications that are being monitored and any calculations that are made. For instance, $spec$ represents the current specification that we are analyzing, while $resp$ represents the response we obtain from performing the actual analysis. Furthermore, the $loop$ of the workflow represents the main component of TVA.

\begin{algorithm}
\caption{TVA Workflow}\label{alg:TVAWorkFlow}
\begin{algorithmic}[1]
\Procedure{Workflow}{}
\State $\textit{spec} \gets \text{the specification to analyze}$
\State $\textit{resp} \gets \text{quantified response from ARIMA analysis}$\\
loop:
\State $resp = analyzeSpecification(spec)$ \label{op:op0}
\If {$resp$ is potentiallyBroken}
\State $makeLatencyEstimate()$
\State $makeCostEstimate()$
\EndIf
\State \textbf{goto} loop
\EndProcedure
\end{algorithmic}
\end{algorithm}

%Now that we have examined the specifics of how our TVA implementation works with both ARIMA and MRA, w

We will next discuss a concrete example that examines the two primary steps of our TVA process as shown in the pseudo code. For this, we will continue to use the self-adaptive hosting service example described in Section \ref{sec: motivatingexample}.

\subsubsection*{\textbf{Step 1: Monitoring Specifications}}

The first step in our TVA approach is to gather and monitor the specifications defined in the SLA. Using the self-adaptive hosting service example, we will assume that it has been configured to record the response time every six seconds. We will also assume that the system's SLA specification defines that a penalty will be incurred if response times do not stay under a 0.7 second threshold. Unfortunately, the majority of self-adaptive processes act in a reactive manner, so the system would not be able to adapt until after the threshold was surpassed. %This can lead to unnecessary scenarios where there system fails to proactively adapt due to it beginning the adaptation process too late. 
Through the application of the time series model ARIMA discussed in this section, we will enable the system to act more proactively by allowing it to anticipate future specification values.


Given the specification and parameters required to make decisions, historical data is used to determine parameters to the ARIMA models (Algorithm~\ref{alg:TVAWorkFlow}, Line~\ref{op:op0}), which provide anticipated future values. For example, in the hosting service when the response time specification is analyzed with ARIMA, the ``response'' is the forecast value. If this forecast value determines that the specification may be broken in the future or is close to being broken, we continue with the rest of our TVA approach.

\subsubsection*{\textbf{Step 2: Tactic Latency and Cost Prediction}}

When the system has determined that it needs to adapt, whether it be because a specification \textit{will} or \textit{may} be broken, our approach then uses regression analysis to predict tactic latency and tactic cost. For example, if our ARIMA analysis from step 1 determines that the hosting service needs to adapt, our TVA approach then predicts tactic latency and cost for all available adaptation tactics. This could entail predicting the latency and cost for a tactic that adds extra computing resources so that response time can be reduced. These predictions are made through a Multiple Regression Analysis (MRA) model. A benefit of focusing on predicting tactic latency and tactic cost is that this can be easily adopted into many existing decision-making processes. For example, one simple option is for the predicted values to merely replace the static, predefined values in the system's decision-making process.%For example, several existing decision making processes consider cost and latency to be a primary concern. Therefore, our approach allows for more informed input into the decision-making process, thus leading to better decisions by the system. 




==> TacticUncertainty-Papers (3)/05-valet.tex <==
\section{VALET: VolAtiLity EmulaTor Tool}
\label{sec: VALETTool}

An additional contribution of this work is the development of the VolAtiLity EmulaTor (\emph{VALET}) tool to generate real-world tactic volatility data to enable the evaluation of our TVA process. While existing datasets such as `The Internet Traffic Archive'\cite{TheInternetTrafficArchive_URL} are commonly used when evaluating self-adaptive processes~\cite{gandhi2014adaptive, dhanapal2017effective}, these are limited as they do not contain an adequate amount of tactic volatility necessary to evaluate our work. To create a sufficient dataset to demonstrate the benefits of TVA, VALET provides tactic volatility data in the form of latency and cost. The tool and generated dataset is available on the project website: \ToolURL

The first action performed in VALET utilizes two physical Raspberry Pi devices, with one acting as the operator and the other as a monitoring instrument. The operator gathers latency data by recording the time required to download an identical 75MB file at one minute intervals, from three different download mirrors around the world. To determine energy usage for this operation, the monitoring instrument collects and records its own energy usage as well as that of the operator. Then, the monitoring Pi calculates the difference between the operating and monitoring Pi's power before and after each download as the overall energy used for the operation. This action provides both real-world latency and cost information. Real-world volatility is also introduced by variations in network speeds that impact the time required to download the file.%\dan{I need to proof this again}\jeff{i proofed this a bit}

The second action performed by VALET obtains an additional form of tactic latency and cost values by performing a `grep' activity. After the file is downloaded, a simple \emph{grep} command searches files contents for a specific string. The amount of time and energy required to perform this task is recorded. %This operation is performed since it emulates not only a system having to gather data, but also searching for the specific data it needs.


%The second \hl{experiment}\dan{operation?} performed in VALET is the grepping \hl{experiments}\dan{operations?}, which obtains an additional tactic latency data through a different kind of file download process. To introduce real-world volatility, VALET downloads an identical zip file from three different locations across the world -- the United States (Boston, MA), Canada (Toronto, ON), and Germany (area unknown). After the file was downloaded, it was unzipped and a simple \emph{grep} command searched the extracted contents for a specific string. This task was performed since it emulates not only a system having to gather data, but also searching for the specific data it needs. Overall, we performed this operation at one minute intervals over the course of an entire day. This created over 1,500 records of tactic latency data. We considered latency to be the time it took to download the file, unzip it, and search its contents.

These operations are performed at one minute intervals over the course of an entire day, creating over 1,400 records of tactic volatility data daily. %We considered latency to be the time it took to download the file, unzip it, and search its contents. 
Figure~\ref{fig:timeseries1} represents a portion of the time series data gathered from our operations, and also visualizes the volatile latency values that we obtained. As shown, the latency times gathered from Germany were quite volatile, with some spikes in volatility in Massachusetts and Ontario download times. 

\begin{figure}[h]
	\centering
     \includegraphics[width=0.9\linewidth]{images/graphStatesV2.png}
    \caption{9-Hour+ Snippet of Latency Data}
    \label{fig:timeseries1}
\end{figure}
%\dan{Cannot read when printed. Converting to Latex}

% What does the feedback for the other paper say
% DK: Remove if space is needed
VALET benefits the software engineering community by enabling developers and researchers to perform evaluations using real-world, time-series data containing tactic volatility. Although VALET represents a specific example of a simple self-adaptive system, the created data is generic enough that it can be used to conduct preliminary evaluations of other machine-learning processes and tactic volatility aware self-adaptive processes.

% Mention how even though this system does specific tasks, the created data is generic enough to be utilized in furtuer systems and evaluations (both of TVA and for other volatility *prediction* systems)


%   this tool which benefits the software engineering community by enabling developers and researchers to perform evaluations using real-world, time-series data containing tactic volatility. Through real-world actions utilizing physical devices, VALET creates robust tactic volatility data in forms of cost and latency volatility. 

%  provides a publicly available dataset containing tactic volatility that will support both researchers and developers of autonomous systems, enabling them to better design and construct systems that will efficiently and effectively operate in dynamic environments.



==> TacticUncertainty-Papers (3)/06-evaluation.tex <==
\section{Evaluation}
\label{sec: Evaluation}

%% Define the RQs
\newcommand{\RQA}{How does not accounting for tactic volatility affect the decision-making process?} 
\newcommand{\RQB}{How effective is ARIMA in allowing the system to monitor system specifications?} 
\newcommand{\RQC}{How effective is MRA in predicting tactic latency and cost at run time?} 
\newcommand{\RQD}{Does using TVA provide substantial improvement to the self-adaptive process over simply using static values for latency and cost?} 

This evaluation addresses the following research questions:

\hangindent=2.5em %\hangafter=1
\textbf{RQ1.} \emph{\RQA} Using the statistical tool R, we demonstrate the negative impact of not accounting for tactic latency volatility and tactic cost volatility in the self-adaptive process.

\hangindent=2.73em %\hangafter=1
\textbf{RQ2.} \emph{\RQB} In our experiments using time series analysis, we demonstrate that time series forecasting with ARIMA helps the system to become more proactive in maintaining specifications defined in the SLA.

\hangindent=2.62em %\hangafter=1
\textbf{RQ3.} \emph{\RQC} In evaluating our multiple regression model, we demonstrate that strong predictive power exists throughout our experiments when estimating tactic latency and cost, even when faced with varying amounts of volatility in the gathered data.

\hangindent=2.47em %\hangafter=1
\textbf{RQ4.} \emph{\RQD} In comparing our approach against existing self-adaptive approaches, such as those that consider tactics to have static latency and cost values, we demonstrate the substantial improvement to the decision-making process that our TVA process provides.

\subsection{\textbf{Experimental Data Analysis}}

To analyze the results found from our VALET experiments, we used the statistical metrics of Root Mean Square Error (RMSE) and Mean Absolute Error (MAE) to evaluate the systematic benefits of our TVA approach. Where $y_i$ is the predicted value and $t_i$ is the actual value at time $i$, RMSE and MAE are defined as:

\begin{equation} 
  		RMSE = [ \sum\limits_{i=1}^{N} (y_i - t_i)^2 / N]^{1/2}
  		\label{eq: rmse}
\end{equation}

\begin{equation} 
  		MAE = \dfrac{\sum\limits_{i=1}^{n} |y_i - t_i|}{n}
  		\label{eq: mae}
\end{equation}

These metrics allowed us to determine TVA's ability to reduce uncertainty and increase the effectiveness of the decision-making process by examining the prediction accuracy of our time series and machine learning models. RMSE provides a better search landscape for determining model parameters and was used to determine how well our models performed in terms of predictive ability, as larger prediction errors become more pronounced due to the squaring of such errors. On the other hand, MAE was used to examine the absolute value of these error differences. MAE was also used for looking at forecasting errors in time series analysis, which is one of its most common uses \cite{mae}.

%\hl{MAE was utilized to measure prediction accuracy, which is common in time series analysis}~\cite{mae}\dan{word this better}.

%\subsubsection*{\textbf{Root Mean Squared Error}} To analyze and further quantify the results found from our experiments, we used the Root Mean Squared Error (RMSE) statistic as a measure of predictive power. Specifically, we used RMSE to quantify prediction error within our response variables, since RMSE puts more weight on larger prediction errors, while also making smaller prediction errors even smaller. RMSE also quantifies this error regardless of the error being in a positive or negative direction.

%\begin{equation} 
%  		RMSE = [ \sum\limits_{i=1}^{N} (y_i - t_i)^2 / N]^{1/2}
%  		\label{eq: rmse}
%\end{equation}
%\vspace{1mm}

%As shown in Equation \ref{eq: rmse}, RMSE represents the quadratic mean of the differences between the estimated values and observed values, or the \textit{residuals}, across multiple testing data points. It serves to aggregate the magnitudes of prediction errors, so the resulting values can be used as a measure of predictive power. Possible values for RMSE range from $0 - \infty$ due to the squared summing of residuals. Therefore, in our analysis, we use RMSE to concretely tell us how our models perform in terms of predictive ability.

%\subsubsection*{\textbf{Mean Absolute Error (MAE)}}

%The final analysis method we used in evaluating our approach is Mean Absolute Error (MAE). Like RMSE, MAE can be used as another measure of predictive power. However, the main difference in these tests is that MAE examines the average absolute error, suggested by its name. 

%\begin{equation} 
%  		MAE = \dfrac{\sum\limits_{i=1}^{n} |y_i - x_i|}{n}
%  		\label{eq: mae}
%\end{equation}

%As shown in Equation \ref{eq: mae}, we can see the main difference between it and RMSE. Where RMSE would take the squared sum of differences over a dataset to determine prediction accuracy, MAE looks at the absolute value of these differences. Furthermore, MAE is much more commonly used when looking at forecasting errors in time series analysis \cite{mae}. Therefore, we use MAE as our measure of prediction accuracy when examining forecasting errors within our ARIMA model.


\subsection{\textbf{Results}}

\noindent \textbf{RQ1: \RQA} We first explored RQ1 by performing a proof of concept evaluation using the statistical tool R, where we emulated the negative effects of poor decision-making by a self-adaptive system. We began by defining two tactics (A $\&$ B) that had arbitrarily defined costs associated with their latency times, where if the tactic took $X$ amount of time to execute, it had $C$ units of cost.

\begin{table}[h]
\begin{center}
\caption{Characteristics of Sample Tactics for Proof of Concept Simulation}
\vspace{2mm}
\label{table: impact}

  \begin{tabular}{ c | c | c | c | c } \hline
 \toprule
  \bfseries & \bfseries Cost & \bfseries Distribution & \bfseries Average & \bfseries SD \\  \midrule 
    \bfseries Tactic A & 5 & Positively Skewed & 3 & 0.5 \\ \hline
    \bfseries Tactic B & 7 & Normal & 3 & 0.5 \\ 
\bottomrule
   \end{tabular}
  \end{center}
\end{table}
\vspace{-1mm}

We next generated a normal distribution and positively skewed distribution with the same mean and standard deviation to represent latency times. We gave the tactic with the higher cost (B) the normal distribution, while the tactic with the lower cost (A) was given the positively skewed distribution. By using two divergent values, we are able to demonstrate the impact of not accounting for tactic volatility in a near-perfect environment (the normal distribution) and in a volatile environment (the positively skewed distribution). It is possible that both latency and cost do not follow these types of distributions, but because they are two extremes, it was sufficient for our proof of concept. Table~\ref{table: impact} shows the characteristics of each tactic.

% Define color for shared items
\definecolor{blue-violet}{rgb}{0.54, 0.17, 0.89}
\definecolor{candypink}{rgb}{0.89, 0.44, 0.48}
\definecolor{ceil}{rgb}{0.57, 0.63, 0.81}
\definecolor{fuzzywuzzy}{rgb}{0.8, 0.4, 0.4}





\begin{figure}[h!]
%\scalebox{.25}
	\centering
%     \resizebox{.7\linewidth}{.5\linewidth}{
%     \resizebox{.7\linewidth}{.5\linewidth}{
	\resizebox{.9\linewidth}{.65\linewidth}{
     
\begin{tikzpicture}
\begin{axis}[
%  title={Overall Cost to System for Executing a Tactic},
  ylabel=Frequency of Cost,
  legend style={font=\fontsize{8.5}{8.5}\selectfont},
%  legend style={nodes={scale=0.5, transform shape},
  xlabel=Cost of executing a tactic, 
  legend image code/.code={
        \draw [#1] (0cm,-0.1cm) rectangle (0.6cm,0.1cm);
    },
]

 \addplot[ybar,bar width=11.5pt,fill=none,opacity=0.8, pattern=horizontal lines] table[col sep=comma,x index=0,y index=1] {data1.txt};\addlegendentry{Tactic A}

 \addplot[ybar,bar width=11.5pt,fill=ceil,opacity=0.6] 
  table[col sep=comma,x index=0,y index=2] {data1.txt};\addlegendentry{Tactic B}

\end{axis}
\end{tikzpicture}
} %Resize box
    \caption{Overall costs of executing a tactic in the R simulations.}
    \label{fig:needForAccountingForVolatility}
\end{figure}

After generating the characteristics of each tactic, we then performed 100 simulations of random sampling from each tactic's latency and multiplied the sampled latency value by its associated cost. This enabled us to build a simulated distribution of ``tactic executions'', where the same tactic is executed every time, but with different latency values. This also allowed us to gather overall cost values that could be used to compare how varying data distributions can impact the predictability of cost for executing a tactic without accounting for any form of volatility.

In our analysis, we found that tactic $B$ may not have had the lowest cost values in the simulations, but it was significantly more consistent (Figure \ref{fig:needForAccountingForVolatility}). However, tactic $B$'s data followed a normal distribution, which is an unlikely occurrence for many real-world systems. Furthermore, even though tactic $A$ had a lower cost of execution with a value of five, it resulted in much more sporadic, and extremely high, overall costs to the system.

%\vspace{2mm}
\noindent \textbf{Outcome:} \textit{Our proof of concept simulations in R successfully demonstrate that accounting for tactic volatility is essential in self-adaptive systems, especially when the system is known to have unpredictable behavior.}


\noindent \textbf{RQ2: \RQB} To evaluate our ARIMA model for time-series forecasting, we used the energy data collected from our VALET tool. Although we had been using a self-adaptive hosting service as an example in this paper, specifically one that monitored response time, the energy usage data is of the same concept. For both, data is gathered over a period of time at equal intervals, thus qualifying it as time-series data. However, the only difference with this analysis is that we did not consider the energy usage when VALET is downloading the file. Therefore, the data used in this research question is strictly the energy usage fluctuations when the device was idle and \textit{not} performing a tactic activity.

To specifically address this research question, we had to loop through the data multiple times to ensure that ARIMA could provide sustainable time-series forecasting predictions. We did this by creating 50 experiments using a randomly selected 90\% portion of our data as training data, and the other 10\% as test data. This type of process can also be seen as a form of \textit{k-cross validation}, which ensures that each data point is included in the training set at least once. After performing this validation, we then calculated both RMSE and MAE values to determine the predictive ability of the ARIMA model.

\begin{figure}[h]
    \centering
	\resizebox{.9\linewidth}{.65\linewidth}{
    
\begin{tikzpicture}
\begin{axis}[
ymin=-0.1, ymax=0.25,
xtick pos=left,
ytick pos=left,
ylabel=MAE Value,
xlabel=Simulation \textit{N}
]
	\addplot[only marks, blue] coordinates {
	(0,0.0807146) (1,0.0713026) (2,0.05549) (3,0.146) (4,0.07891) (5,0.1082) (6,0.08767) (7,0.05549) (8,0.1035863) (9,0.090701) (10,0.15396) (11,0.118238) (12,0.103863) (13,0.047307) (14,0.05549) (15,0.123976) (16,0.0943001) (17,0.080716) (18,0.0709601) (19,0.077146) (20,0.06607) (21,0.0713076) (22,0.0803746) (23,0.06401) (24,0.07282) (25,0.06978) (26,0.079281) (27,0.0637641) (28,0.06958) (29,0.11878) (30,0.117531) (31,0.0667258) (32,0.06926) (34,0.06696) (35,0.1534396) (36,0.0676496) (37,0.1181738) (38,0.07146) (39,0.027546) (40,0.1196) (41,0.0943601) (42,0.06031) (43,0.060376) (44,0.15896) (45,0.055849) (46,0.078282) (47,0.11101) (48,0.075258) (49,0.07281)};\addlegendentry{HMM}
	
	\addplot[only marks, mark=o,draw=black, red] coordinates {
	(0,0.05629) (1,0.04103) (2,0.04332) (3,0.1046) (4,0.06321) (5,0.07871) (6,0.066720) (7,0.04412) (8,0.06899) (9,0.03029) (10,0.0987) (11,0.07152) (12,0.06113) (13,0.02363) (14,0.03243) (15,0.07598) (16,0.065563) (17,0.05397) (18,0.03456) (19,0.05563) (20,0.0602) (21,0.04332) (22,0.075563) (23,0.05661) (24,0.044503) (25,0.044879) (26,0.05234) (27,0.033289) (28,0.02236) (29,0.09956) (30,0.09112) (31,0.04631) (32,0.02223) (34,0.0510) (35,0.101123) (36,0.04663) (37,0.09445) (38,0.04976) (39,0.0156) (40,0.10112) (41,0.051238) (42,0.04361) (43,0.031126) (44,0.1098) (45,0.04629) (46,0.066731) (47,0.07134) (48,0.059713) (49,0.03164)};\addlegendentry{ARIMA}
    
    \draw[ultra thick, black] (axis cs:\pgfkeysvalueof{/pgfplots/xmin},0) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},0);
    
\end{axis}
\end{tikzpicture}

 } % Resize box

\caption{MAE Values Over 50 Experiments Using ARIMA vs HMM for Time Series Forecasting}
\label{fig:maeHMM}
% it doesnt demonstrate anything, its just purely a plot of what we saw. Because the simulations are independent you cant draw any conclusions from it, so it's purely for visualization

\end{figure}

Figure \ref{fig:maeHMM} shows the MAE results from our ARIMA model compared to a previously used Hidden Markov Model (HMM). Each simulation was independently performed, so no patterns should be inferred from the left to right sequence. Over the course of the experiments we saw fairly stable MAE values, represented by the small range between the lowest MAE value and the highest. Furthermore, the ARIMA model was not only successful by itself, but also better than that of the HMM model. We believe this occurred as we did not have enough features in our model to allow for a full treatment of a HMM.

%Since each experiment in our evaluation is independent from the others, no patterns should be inferred nor concluded from the graph. For example, from roughly simulation 20 to 40 the MAE values for the HMM model form a near horizontal line. However, this does not mean there are any underlying reasons for this. The same 50 experiments could be run again and the shape of the graph could look entirely different. What we care about most in the graph is how wide the ``spread" of these MAE values are, as this tells us how stable our predictions were. Over the course of the experiments in Figure \ref{fig:maeHMM} we saw fairly stable MAE values, represented by the small range between the lowest MAE value and the highest. Furthermore, not only were MAE values consistent but they were also considerably low. Therefore, this tells us that the predictive ability of our model was both strong and consistent across all the data we gathered.

\begin{figure}[h]
    \centering
%	\resizebox{.6\linewidth}{.45\linewidth}{
	\resizebox{.9\linewidth}{.65\linewidth}{
    
\begin{tikzpicture}
\begin{axis}[
ymin=-0.1, ymax=0.25,
xtick pos=left,
ytick pos=left,
ylabel=RMSE Value,
xlabel=Simulation \textit{N}
]
	\addplot[only marks, blue] coordinates {
	(0,0.14420) (1,0.09424) (2,0.06012) (3,0.1972) (4,0.09712) (5,0.1253) (6,0.09015) (7,0.04263) (8,0.13356) (9,0.1178) (10,0.1759) (11,0.13354) (12,0.12236) (13,0.03231) (14,0.04489) (15,0.1597) (16,0.11463) (17,0.09765) (18,0.088746) (19,0.09856) (20,0.04923) (21,0.088163) (22,0.09971) (23,0.04463) (24,0.088963) (25,0.0496) (26,0.05913) (27,0.04480) (28,0.06623) (29,0.15630) (30,0.13412) (31,0.07123) (32,0.07503) (34,0.04320) (35,0.19783) (36,0.051261) (37,0.148913) (38,0.05597) (39,0.039336) (40,0.14879) (41,0.11603) (42,0.04931) (43,0.05594) (44,0.18936) (45,0.051023) (46,0.071136) (47,0.14593) (48,0.07176) (49,0.06314)};\addlegendentry{HMM}
	
	\addplot[only marks, mark=o,draw=black, red] coordinates {
	(0,0.07130) (1,0.0546) (2,0.03630) (3,0.09136) (4,0.05496) (5,0.06981) (6,0.046720) (7,0.08412) (8,0.03899) (9,0.0209) (10,0.08337) (11,0.07832) (12,0.04326) (13,0.02033) (14,0.02213) (15,0.11563) (16,0.07891) (17,0.05012) (18,0.03563) (19,0.054413) (20,0.07113) (21,0.04132) (22,0.08801) (23,0.06332) (24,0.04195) (25,0.07713) (26,0.05103) (27,0.03190) (28,0.02173) (29,0.1173) (30,0.11083) (31,0.04133) (32,0.02116) (34,0.0679) (35,0.1350) (36,0.04165) (37,0.11732) (38,0.09713) (39,0.0190) (40,0.13013) (41,0.04109) (42,0.0389903) (43,0.029948) (44,0.1271) (45,0.04103) (46,0.07821) (47,0.09463) (48,0.054522) (49,0.02693)};\addlegendentry{ARIMA}
    
    \draw[ultra thick, black] (axis cs:\pgfkeysvalueof{/pgfplots/xmin},0) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},0);
    
\end{axis}
\end{tikzpicture}

}

\caption{RMSE values over 50 experiments using ARIMA vs HMM for Time Series Forecasting}
\label{fig:rmseHmmArima}

\end{figure}

As discussed previously, larger prediction errors will become more pronounced and smaller prediction errors will become less pronounced when using RMSE. Due to this, we expected the RMSE graph to be slightly more dispersed compared to MAE. In examining the RMSE differences between HMM and ARIMA, we found exactly this. Looking at Figure \ref{fig:rmseHmmArima} closely, we can see how the RMSE values have more variation than the MAE values in Figure \ref{fig:maeHMM}. However, this does not mean there was less predictive power or that the model is less useful. We report on both to show the differences in possible inferences. For example, in applying our TVA technique the system's engineers may care more about larger prediction errors; deeming RMSE a more powerful statistic for determining predictive ability of their models. Conversely, if the system's engineers want more of a ``man-in-the-middle'' statistic, they may deem MAE more appropriate. For our experiments, using RMSE or MAE would lead to the same conclusion -- both statistics clearly favor the ARIMA model over the HMM model for time series forecasting.

%\vspace{2mm}
\noindent \textbf{Outcome:} \textit{Through an evaluation process using time series data, TVA demonstrated it's ability to positively support proactive adaptations.}\\


%allow for proactive adaptations. TVA accomplishes this by applying an ARIMA time series model to predict future values for specifications, thus allowing the system to start adapting before they may become broken.}


\noindent \textbf{RQ3: \RQC} Unpredictability is considered to be an undesirable trait of a self-adaptive system and is frequently associated with much of the uncertainty that surrounds self-adaptive systems~\cite{rodrigues2018learning, tomforde2016organic, Kinneer2018ManagingUI, esfahani2014management}. To determine how well TVA can improve the predictability of a self-adaptive system, we examined the prediction errors across our tactic latency data and our tactic cost data. For space considerations and the use of RMSE being more appropriate in this context, this research question does not report MAE values.

%To determine how well TVA can improve the predictability of a self-adaptive system, we examined how well the ground truth feature weights were estimated with our BRR model and how accurate our estimates of tactic latency and cost were. For the feature weight estimation, the closer we are to the ground truth, the better the model is at making predictions, thus reducing uncertainty. To quantify how well BRR can perform, we looked at MAE values for the feature weight estimation and RMSE values for the prediction errors of our response variables, i.e. latency and cost.

Unlike RQ \#2 where we only examined the energy usage for when the Raspberry Pi was idle, RQ \#3 only examined the energy usage when the device \textit{was} performing the file download. If we had used the energy usage data from when the device was idle, our models would have been invalid. This is because the file download represented a tactic of gathering more information, thus any energy data gathered while the device was idle did not represent tactic latency.

\begin{figure}[h]
    \centering
%	\resizebox{.6\linewidth}{.45\linewidth}{
 	\resizebox{.9\linewidth}{.65\linewidth}{
 	
\begin{tikzpicture}
\begin{axis}[
ymin=-0.1, ymax=0.25,
xtick pos=left,
ytick pos=left,
ylabel=RMSE Value,
xlabel=Simulation \textit{N}
]
	\addplot[only marks, blue] coordinates {
	(0,0.104526215611) (1,0.09663001) (2,0.0651396100502) (3,0.088610036) (4,0.1199093) (5,0.0979030) (6,0.0752027817414) (7,0.088082200573) (8,0.125437336115) (9,0.0777104) (10,0.0601853376522) (11,0.0777109489224) (12,0.0601853376522) (13,0.0649311136285) (14,0.104526215611) (15,0.0651396100502) (16,0.067980046989) (17,0.0691105310622) (18,0.104526215611) (19,0.0691105310622) (20,0.0777109489224) (21,0.104526215611) (22,0.0491833826094) (23,0.067980046989) (24,0.113685402858) (25,0.0777109489224) (26,0.0491833826094) (27,0.067980046989) (28,0.113685402858) (29,0.0691105310622) (30,0.067980046989) (31,0.0449456839679) (32,0.0491833826094) (33,0.066531787513) (34,0.066531787513) (35,0.100268434489) (36,0.104526215611) (37,0.0719623111926) (38,0.0740933208235) (39,0.0925966318751) (40,0.0752655663011) (41,0.0691105310622) (42,0.067980046989) (43,0.0740933208235) (44,0.0740933208235) (45,0.0752655663011) (46,0.088082200573) (47,0.0752027817414) (48,0.0601853376522) (49,0.0807571593297)
	};\addlegendentry{BRR}
    
    \addplot[only marks, mark=o,draw=black, red] coordinates {
    (0,0.07953) (1,0.04623) (2,0.04113) (3,0.05693) (4,0.0717930) (5,0.06593) (6,0.071394) (7,0.055930) (8,0.11036) (9,0.046179) (10,0.053910) (11,0.071063) (12,0.0469003) (13,0.0556971) (14,0.123609) (15,0.053608) (16,0.033691) (17,0.065960) (18,0.088913) (19,0.063120) (20,0.0700356) (21,0.12230) (22,0.0407993) (23,0.063061) (24,0.099861) (25,0.0699789) (26,0.045630) (27,0.064430) (28,0.099730) (29,0.061130) (30,0.0667933) (31,0.0401136) (32,0.0412369) (33,0.0601137) (34,0.051306) (35,0.05913) (36,0.066971) (37,0.05710310) (38,0.0633719) (39,0.075906) (40,0.0704462) (41,0.0679003) (42,0.06113086) (43,0.0411036) (44,0.05103791) (45,0.05930036) (46,0.071393) (47,0.0477913) (48,0.0399713) (49,0.0665130)
	};\addlegendentry{MRA}
    
    \draw[ultra thick, black] (axis cs:\pgfkeysvalueof{/pgfplots/xmin},0) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},0);
    
\end{axis}
\end{tikzpicture}

}

\caption{RMSE Values for Tactic Cost Predictions of MRA vs BRR}
\label{fig:rmseCostValet}

\end{figure}

%As demonstrated in Figure~\ref{fig:brrRasPi}, we found that using MRA performed well for estimating the ground truth feature weights in the tactic latency model -- demonstrated by the overlapping plots. We observed the most significant performance from our model when the ground truth weights began to deviate away from zero, whether it be small or large deviations. This is further supported by the resulting MAE value of 0.042707 from our experiments. Additionally, being able to better estimate feature weights that deviated away from zero did not hinder the model's ability to estimate other feature weights.

%Due to the success of our BRR model in feature weight estimation, it was of no surprise how it performed in its predictive ability of tactic latency and tactic cost. Like we did with Research Question \#1, evaluating the BRR model also took a series of 50 experiments, where after each experiment we calculated RMSE values to determine it's predictive ability. However, as stated previously, this research question uses RMSE to look at the differences between estimated response output and actual response output.

Figure \ref{fig:rmseCostValet} demonstrates why MRA is more appropriate for TVA. Over the course of the 50 simulations, MRA reported lower RMSE values than BRR in almost every case. In cases where BRR did outperform MRA, the differences were fairly negligible. However, the plots are closer together than what we would have initially expected. We believe this was caused by only having a few cases of extreme volatility in the cost data, therefore not allowing the two models to really differentiate themselves.  

\begin{figure}[h]
    \centering
%	\resizebox{.6\linewidth}{.45\linewidth}{
	\resizebox{.9\linewidth}{.65\linewidth}{
    
\begin{tikzpicture}
\begin{axis}[
ymin=-0.1, ymax=0.25,
xtick pos=left,
ytick pos=left,
ylabel=RMSE Value,
xlabel=Simulation \textit{N}
]
	\addplot[only marks, blue] coordinates {
	(0,0.124746) (1,0.0746) (2,0.049) (3,0.1396) (4,0.1382) (5,0.146082) (6,0.03001267) (7,0.0849) (8,0.103511827663) (9,0.09401) (10,0.126) (11,0.07838) (12,0.10663) (13,0.15267) (14,0.0239) (15,0.05156) (16,0.0233701) (17,0.09467) (18,0.031) (19,0.0746) (20,0.0721) (21,0.114746) (22,0.084746) (23,0.0341) (24,0.1285) (25,0.09258) (26,0.0591) (27,0.0958) (29,0.11838) (30,0.05031) (31,0.0258) (32,0.0258) (33,0.1096) (34,0.0496) (35,0.082496) (36,0.112296) (37,0.0838) (38,0.0846) (39,0.06146) (40,0.09986) (41,0.0701) (42,0.15641) (43,0.0441) (44,0.09896) (45,0.13849) (46,0.1182) (47,0.10431) (48,0.08258) (49,0.0481)};\addlegendentry{BRR}
    
    \addplot[only marks, mark=o,draw=black, red] coordinates {
    (0,0.088193) (1,0.0423360) (2,0.044160) (3,0.088693) (4,0.09799) (5,0.100893) (6,0.030113) (7,0.057719) (8,0.06663) (9,0.0571411) (10,0.08893) (11,0.044976) (12,0.091130) (13,0.107910) (14,0.020119) (15,0.039970) (16,0.021126) (17,0.077913) (18,0.0255617) (19,0.0577963) (20,0.0510030) (21,0.0771682) (22,0.05813645) (23,0.0307947) (24,0.0812409) (25,0.0705581) (26,0.041130) (27,0.062405) (29,0.076810) (30,0.04630) (31,0.021130) (32,0.022003) (33,0.071993) (34,0.0400191) (35,0.06003215) (36,0.077506) (37,0.0511360) (38,0.0700363) (39,0.04822613) (40,0.0617752) (41,0.05722036) (42,0.1033608) (43,0.0399613) (44,0.08100231) (45,0.0911963) (46,0.07339192) (47,0.0601123) (48,0.0643520) (49,0.03881095)
	};\addlegendentry{MRA}
    
    \draw[ultra thick, black] (axis cs:\pgfkeysvalueof{/pgfplots/xmin},0) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},0);
    
\end{axis}
\end{tikzpicture}

}

\caption{RMSE values for tactic latency predictions of MRA vs BRR}
\label{fig:rmseLatencyValet}

\end{figure}

As shown in Figure \ref{fig:rmseLatencyValet}, we observed very similar results between the RMSE values calculated for tactic latency predictions and those calculated for tactic cost. In most cases, prediction errors with MRA were much smaller than those of BRR, and in examining the figures closely, the differences in volatility that were experienced can be observed. As mentioned previously, there were not as many extreme cases of volatility in the tactic cost data. However, within the tactic latency data we saw many cases of volatility, with some cases being extreme. This can partially be seen in Figure \ref{fig:rmseLatencyValet} since more volatility will likely lead to larger prediction errors. Thus, it came at no surprise that the RMSE values for tactic latency had a wider-spread than those associated with tactic cost. 

In order to say the MRA model can be generalized to other data sets for predicting tactic latency and cost, observing consistent RMSE values regardless of the data it was modeling was imperative. Figure \ref{fig:rmseCostValet} and Figure \ref{fig:rmseLatencyValet} demonstrate that not only were RMSE values low for both data sets, but the values were stable. Therefore, MRA was able to handle the volatile latency data and cost data collected for these experiments when making its predictions. 

%\vspace{2mm}
\noindent \textbf{Outcome:} \textit{The RMSE results gathered from addressing this research question demonstrate that MRA is able to handle tactic volatility when predicting tactic latency and cost. Throughout our experiments, MRA consistently provided stable predictive power, even in the presence of volatile data.}


\noindent \textbf{RQ4: \RQD} Thus far, we have demonstrated the benefits of using an ARIMA time series model and a MRA model in a self-adaptive process to predict tactic latency and cost, while also maintaining specifications defined in the SLA. However, to provide further confidence in our TVA approach, we also compared it to current self-adaptive processes. Since current processes consider tactic latency and cost to be static values, there is no one specific work that TVA can be compared to. Rather, for this research question, we compared the results from our approach to what we consider the ``baseline'' model defined below:

\begin{framed}
\textit{\textbf{Baseline Model}: A model that uses a simple average of previous tactic latency and cost values as its prediction process for estimating future tactic behavior.}
\end{framed}

While utilizing the average value for latency and cost values may seem like a naive comparison, in many cases it can be a be a strong predictor especially when compared a static value (as in other current self-adaptive processes) on a dynamic time series. Similar to RQ \#2, we will also report the MAE and RMSE values for model comparison.

%As with RQ \#2, we also report both MAE and RMSE values for model comparison.\dan{Kind of a weak ending to this paragraph. Where are these values going to be reported?}

%Although examining the average for previous latency and cost values may seem like a naive comparison, this provides us with a better comparison than using a static value like current self-adaptive processes. This is because doing something as simple as taking the average of a given set of latency values can provide more predictive ability and information than considering latency to be a static value for every execution. This also takes out any ambiguity or subjectivity in defining what the static value should be for comparison. Therefore, comparing our TVA process to taking the average of previous values is appropriate for evaluation purposes. As with Research Question \#2, we also report both MAE and RMSE values for model comparison.

\begin{figure}[h]
    \centering
%	\resizebox{.6\linewidth}{.45\linewidth}{
	\resizebox{.9\linewidth}{.65\linewidth}{	
    
\begin{tikzpicture}
\begin{axis}[
%ymin=-0.1, ymax=0.25,
xtick pos=left,
ytick pos=left,
ylabel=RMSE Value,
xlabel=Simulation \textit{N}
]
	\addplot[only marks, blue] coordinates {
	(0,0.4679022) (1,0.3178) (2,0.3155) (3,0.2469) (4,0.4356) (5,0.33728) (6,0.2316) (7,0.48687) (8,0.42289) (9,0.4382) (10,0.4956) (11,0.2344) (12,0.4001) (13,0.3420) (14,0.4199) (15,0.49354) (16,0.4585) (17,0.3970) (18,0.3162) (19,0.4442) (20,0.3586) (21,0.43581) (22,0.3232) (23,0.3857) (24,0.3706) (25,0.4734) (26,0.4482) (27,0.32721) (28,0.4577) (29,0.48418) (30,0.25178) (31,0.387339) (32,0.4498) (33,0.4904) (34,0.4942) (35,0.3666) (36,0.38681) (37,0.46701) (38,0.30941) (39,0.3854) (40,0.4855) (41,0.40154) (42,0.2802) (43,0.27649) (44,0.43867) (45,0.42811) (46,0.4040) (47,0.30126) (48,0.45843) (49,0.30499) };\addlegendentry{TVA}
    
    \addplot[only marks, mark=o,draw=black, red] coordinates {
    (0.6066) (1,0.5481) (2,0.52841) (3,0.72919) (4,0.5445) (5,0.6743) (6,0.56503) (7,0.63325) (8,0.54903) (9,0.61590) (10,0.4756) (11,0.5333) (12,0.51868) (13,0.72003) (14,0.5234) (15,0.67793) (16,0.4866) (17,0.72304) (18,0.704710) (19,0.72784) (20,0.79789) (21,0.7173) (22,0.66314) (23,0.78829) (24,0.49865) (25,0.76610) (26,0.66190) (27,0.52240) (28,0.6573) (29,0.49610) (30,0.72732) (31,0.66288) (32,0.4350913) (33,0.59541) (34,0.48901) (35,0.51190) (36,0.56188) (37,0.52642) (38,0.43569) (39,0.578414) (40,0.41275) (41,0.47245) (42,0.5378) (43,0.673521) (44,0.72538) (45,0.55426) (46,0.7183510) (47,0.780043) (48,0.461672) (49,0.79306)
    };\addlegendentry{Baseline}

    
\end{axis}
\end{tikzpicture}

}

\caption{Baseline Value Approach vs TVA - RMSE Differences}
\label{fig:rmseComparisons}

\end{figure}

As shown in Figure \ref{fig:rmseComparisons}, TVA was able to obtain substantially lower RMSE values. In comparison, TVA had an average RMSE value of 0.0396 while the baseline approach had an average RMSE value of 0.0694. Also represented in this diagram is the ability of TVA to handle volatility. While the spread of RMSE values remained fairly consistent for TVA, the baseline approach saw a much wider spread; a direct result of only using a static value for latency and cost. Although there were cases where the baseline approach did outperform TVA (7 in total of 50 experiments), the differences in these values were fairly negligible. 

\begin{figure}[h]
    \centering
%	\resizebox{.6\linewidth}{.45\linewidth}{
	\resizebox{.9\linewidth}{.65\linewidth}{
    
\begin{tikzpicture}
\begin{axis}[
%ymin=-0.1, ymax=0.25,
xtick pos=left,
ytick pos=left,
ylabel=MAE Value,
xlabel=Simulation \textit{N}
]
	\addplot[only marks, blue] coordinates {
	(0,0.42090) (1,0.31469) (2,0.34992) (3,0.27745) (4,0.3742) (5,0.30119) (6,0.2906) (7,0.41035) (8,0.38942) (9,0.399682) (10,0.47163) (11,0.318643) (12,0.42463) (13,0.3655) (14,0.3940) (15,0.46712) (16,0.4306) (17,0.38132) (18,0.33978) (19,0.42103) (20,0.36713) (21,0.41863) (22,0.34012) (23,0.37620) (24,0.35203) (25,0.441003) (26,0.41064) (27,0.376403) (28,0.42643) (29,0.44970) (30,0.29761) (31,0.35360) (32,0.410793) (33,0.44039) (34,0.4642) (35,0.386460) (36,0.33025) (37,0.42273) (38,0.324692) (39,0.36024) (40,0.45973) (41,0.391630) (42,0.316098) (43,0.307913) (44,0.41309) (45,0.38961) (46,0.39972) (47,0.336412) (48,0.42016) (49,0.37340) };\addlegendentry{TVA}
    
    \addplot[only marks, mark=o,draw=black, red] coordinates {
    (0.55430) (1,0.51306) (2,0.48790) (3,0.61913) (4,0.49873) (5,0.62136) (6,0.54063) (7,0.57959) (8,0.521033) (9,0.58716) (10,0.4506) (11,0.51033) (12,0.49760) (13,0.65493) (14,0.500178) (15,0.63306) (16,0.47790) (17,0.67492) (18,0.66513) (19,0.60719) (20,0.621303) (21,0.5888130) (22,0.533261) (23,0.65709) (24,0.48893) (25,0.621396) (26,0.64469) (27,0.51103) (28,0.63688) (29,0.48996) (30,0.655643) (31,0.62163) (32,0.422130) (33,0.56310) (34,0.46604) (35,0.510996) (36,0.544306) (37,0.500397) (38,0.411036) (39,0.555973) (40,0.400613) (41,0.4557136) (42,0.4976310) (43,0.62106) (44,0.65971) (45,0.52230) (46,0.579162) (47,0.6010396) (48,0.45269) (49,0.7198703)
    };\addlegendentry{Baseline}

    
\end{axis}
\end{tikzpicture}

}

\caption{Baseline Value Approach vs TVA - MAE Differences}
\label{fig:maeComparisons}

\end{figure}


In examining the MAE values shown in Figure \ref{fig:maeComparisons}, we found that MAE did not behave as we expected. In RQ \#2, it is fairly evident that RMSE made larger prediction errors larger, and smaller prediction errors smaller. However, in this research question, those kinds of results are not as evident. In examining the MAE values from TVA, we can see the plot is a bit more condensed than then RMSE plot, but the MAE values for the baseline model did not follow the same trend as strongly. We believe this occurred because the baseline model's prediction method was extremely poor, justified by both the RMSE and MAE plots. Regardless, TVA was still superior in predictive ability compared to the baseline model.

\vspace{0mm}
\noindent \textbf{Outcome:} \textit{These findings demonstrate that TVA is beneficial for decision-making processes in self-adaptive systems, and offer a significant improvement over assuming tactic latency and tactic cost to be static values.}


==> TacticUncertainty-Papers (3)/07-threats.tex <==
\section{Threats and Future Work}
\label{sec: threats}

Our evaluations have demonstrated TVA's ability to enable systems to better account for tactic volatility. However, there are limitations to this work. In many systems, tactic cost may be an ambiguous and tough-to-define measurement. This inability to accurately measure cost could inhibit the adoption of our process by limiting the quality and quantity of observed input values into our prediction process. Furthermore, cost can also be a relative term, and in our TVA approach we consider it to be a quantifiable value. For example, one could argue that the `cost' for performing an action could be the wear and tear on a physical component in the device. Such cost is difficult to quantify in most situations. Therefore, when using TVA the notion of cost must be restricted to a value that is reasonably easy to quantify.

Although TVA provides a method of monitoring specifications defined in the SLA, not all specifications are necessarily measurable with time-series analysis. For example, a system may have the specification that it must be available 99.99\% of the time. This is not something that could be measured or predicted using time-series analysis, rather it would need to be accounted for using fault detection techniques in the system's architecture. In systems that do not directly utilize a SLA, the improved tactic estimations can still be used to benefit the decision-making process by providing more informed and accurate tactic attribute values. Future work should be conducted to examine precisely how our TVA process can be incorporated into these systems and determine the benefits that they will have.


%\hl{In systems that may not directly utilize a SLA, the improved tactic estimations can still be used to benefit the decision-making process of these systems as well. Future work should be conducted to examine precisely how our TVA process can be incorporated into these systems and determine the benefits that they will have.}\dan{Need to rewrite this entire section}


% \hl{In systems that may not directly utilize a SLA, the improved tactic estimations can still be included in the decision-making process of these systems. Future work should be done to examine precisely now our TVA process can be incorporated into these systems and determine the benefits that they will have. However based on our initial findings, we are confident that our process of accounting for tactic volatility would be beneficial to these systems as well.}\dan{Added}

To be completely proactive, future work must be done to update our ARIMA method to consider tactic latency. Currently, this process can alert the system of a specification that is about to be broken, however the time between monitoring intervals may not leave enough time to fully execute a tactic. Therefore, there may be occurrences where specifications are slightly broken for a period of time. This future work will likely examine other time series models as well that can be flexible to different systems and datasets. This in turn would also help us to start addressing the problem of not having enough data to build other kinds of models and would allow this work to develop into an entire decision-making framework.

%% Future Work
Although we have demonstrated the benefits of our TVA approach with real-world experimental data, we have yet to implement TVA on any physical devices. Future work will consist of including our adaptation process into physical equipment such as IoT devices, small unmanned aerial vehicles (UAV), and self-adaptive web systems. 
% Future work should also be conducted to understand 

ARIMA demonstrated its ability to perform time series forecasting, however no mechanisms are in place to quantify uncertainty within these predictions. Future work could be done to include confidence intervals around predictions made by ARIMA. For example, instead of only predicting a single point value for a specification, we could predict a range that states something such as the following, ``\textit{we are 95\% certain response time will be between 3.1 and 3.7 seconds}''. This would allow the system to have a ``buffer'' zone around its predictions, therefore providing the decision-making process with more information.

Additionally, the ARIMA models utilized in this work were pre-trained on gathered historical data. It is also possible to have the ARMIA models be updated online as new data is gathered by a system to adapt themselves as more information becomes available. Other methods for time series prediction such as recurrent neural networks (RNNs), which have been successfully used for a variety of time series forecasting problems~\cite{di2016artificial,maknickiene2012application,gers-lstm-forget-2000,felder2010wind,choi2015doctor,elsaid2018optimizing,elsaid2019evolving}, can be examined as well. RNNs may also potentially be able to incorporate non-time series data into predictions.


%Now that we have shown the benefits of not using static values for tactic latency and cost, future work must be done to compare TVA to more machine-learning and time-series forecasting models. In this investigation some of the important factors to examine may be: computing resources (as more complex machine-learning models will tend to require more computational resources) and models that perform well regardless of the availability of data. Furthermore, examining the use of time series models that have ''longer memory" should also be examined to determine the concrete differences between the two and their possible uses in self-adaptive systems. 


Our evaluation data was created using two Raspberry Pi's, and does not simulate a complicated system such as a self-driving car or a UAV. However, this generated data was intended to help demonstrate the capabilities of TVA and the benefits of accounting for tactic volatility. In reality, the data generated by these tools could represent virtually any form of tactic volatility (\eg the time required for a UAV to communicate with a base station or the energy cost of a self-driving car performing a tactic).

There are a few potential limitations to the use of our VALET tool and dataset in the evaluation of our proposed TVA process. First, VALET generates its data by performing a small number of tasks. A real-world self-adaptive system would likely perform a large number of tasks in any given adaptation, which depending on the system, could impact one another. VALET is also limited in the forms of variability that it may encounter as opposed to a real-world system. For example, VALET is significantly less likely to be actively targeted by human hackers than many real-world self-adaptive systems, which could limit the encountered variability. However, it is somewhat unreasonable to expect that any created evaluation system would have the capabilities to address a majority of real-world events and possibilities. Despite these possible limitations, we are confident in the ability of VALET in creating satisfactory evaluation data for not only our study, but for future research conducted by others.



==> TacticUncertainty-Papers (3)/08-conclusions.tex <==
\section{Conclusion}
\label{sec: conclusion}
In this work, we propose a Tactic Volatility Aware (TVA) process that is able to account for tactic volatility in multiple ways. TVA first uses time-series forecasting with an autoregressive integrated moving average (ARIMA) model to monitor system specifications defined in the SLA, supporting the system in acting more proactively while maintaining them. Next, TVA uses multiple regression analysis (MRA) to predict tactic latency and cost helping to improve the decision-making process. Our contribution also includes a tool that utilizes physical devices to create real-world tactic volatility data.


% This toola and dataset are available on th e


%As the world begins to use more and more autonomous systems everyday, addressing tactic volatility must become a first-class concern. Without this ability, systems will not be able to perform at their peaks, possibly resulting in severe consequences. 


==> TacticUncertainty-Papers (3)/09-acknowledgements.tex <==
\section*{Acknowledgements}
Elements of this work are sponsored by the United States Air Force Research Laboratory (AFRL). 


==> TacticUncertainty-Papers (3)/problemdef.tex <==
Despite the growing emphasis on accounting for uncertainty in self-adaptive systems~\cite{moreno2016efficient, camara2017reasoning, esfahani2013uncertainty, moreno2018uncertainty}, it has not been addressed at a tactic decision-making process level. Examples of tactic uncertainties, along with motivating examples for them, are described in this section.

% Put into a separate file

% Give some examples of tactic volatility. Perhaps do simulations of leading existing systems to demonstrate that how ?
% Discuss how this could negative impact the system
% >>> Cut down on this from the ASE paper

%\dan{Thurs: Do this}

%Self-adaptive systems typically operate in non-deterministic environments, where the system will encounter numerous unforeseeable events and scenarios. The actions taken by self-adaptive systems will also frequently encounter different forms of volatility, many of which will substantially impact the system's ability to main efficient, and effective. Some forms of volatility include:



% Take much of this from the YIP
\jeff{If we end up running out of room I think the problem definition section could be more concise}
\subsection{Tactic Latency}
The amount of time required to implement a tactic is known as \emph{tactic latency}. Due to various circumstances, these latency times can sometimes become highly volatile. One example tactic could be to access information from a remote server, whose latency time could be volatile due to network or server congestion. As a result, this prevents the system from accurately predicting the behavior of a tactic. Previous works have shown that latency aware algorithms offer several advantages compared to those that do not consider latency~\cite{camara2014stochastic, esfahani2013learning}. However, due to the unpredictable nature of many tactics, their latency times cannot always be accurately estimated. Unfortunately, existing work conducted on decision-making processes in self-adaptive systems also considers tactic latency to be a predetermined, static value. When a system is not able to account for tactic latency volatility or `learn' from previous implementations about what this value may possibly be, this creates uncertainty in the decision making process.  

\subsubsection*{\bfseries Example: Latency Volatility in UAVs}

An unmanned aerial vehicle (UAV), is often used in reconnaissance missions in order to keep soldiers out of harms way. As an example, there may be times when a UAV is flying over an area to locate a certain person with a main goal of taking hi-resolution photos of the area once the person is potentially located. In a scenario where the UAV identities the possible target, several steps must be taken. For this example, we will assume that the UAV needs to physically prepare the camera for taking photos and will need to communicate with the base station while performing other necessary calculations (planned time of .2 seconds). This anticipated latency time means that the UAV should plan on beginning the photography process .2 seconds before it is within range of the possible target. However, in the event of poor weather conditions or something similar, it could take the UAV .4 seconds to communicate with the base station and receive the required data. This would result in the UAV missing its target window for photographing the area, and possibly miss identifying the target entirely. If the UAV was able to use previous knowledge about its prior mission experiences with communication lag, it would enable the UAV to account for tactic latency volatility, further improving the decision-making process for the next time adaptation is required. This example scenario is shown in Figure~\ref{fig:UAVLatencyExampleCamera}. 

\begin{figure*}[ht]
	\centering
    \includegraphics[scale=1.05]{images/UAVCameraExample.PNG}
    \caption{Impact of Unexpected Latency in UAV}
    \label{fig:UAVLatencyExampleCamera}
\end{figure*}




\subsection{Tactic Dependability}
%\subsection{\textbf{Tactic Dependability}} 

In a self-adaptive system certain tactics may be more dependable than others, and having knowledge of this is crucial for the decision-making process. The measure of how well a tactic correctly produces its expected functionality is known as \emph{tactic dependability}. Due to numerous reasons, tactics may sometimes fail to produce their expected results leading to extra consumption of resources or even disastrous consequences in some cases. Therefore, having the ability to estimate when a tactic may or may not work properly is imperative for a self-adaptive system to remain dependable. 
    
\subsubsection*{\bfseries Example: Dependability Volatility in Cloud}

In a cloud-based system, there may be times where interaction with remote computers is required for retrieving necessary information or to make an API call. Due to various reasons, the connection to these remote resources may be inhibited by network congestion or even cyberattacks. Regardless of how well the connections have worked in the past, there will be times where the system attempts to connect to one of the remote computers and gets an unexpected result. For instance, the tactic that connects to a remote computer may only return the expected result 80\% of the time, while the API-call tactic may only return the expected result 90\% of the time. Not being able to account for this in the decision-making process could lead to the system attempting to access the same remote resources every time, even though a similar more dependable resource may be available. 

Figure~\ref{fig:CloudDependabilityExample} displays a possible scenario where a system has three tactic options with identical costs, but with various amounts of produced utility and levels of dependability. If the dependability of each tactic is the same, then selecting the most appropriate tactic is fairly simple; select the one with the highest estimated utility. However, as shown in Figure~\ref{fig:CloudDependabilityExample}, when the dependability and utility of each possible tactic differs, the system must have a way to weigh these differences in order to determine which tactic is most appropriate.

\begin{figure}[h]
	\centering
    \includegraphics[scale=0.85]{images/trade-off.PNG}
    \caption{Impact of Dependability Uncertainty}
    \label{fig:CloudDependabilityExample}
\end{figure}


==> TacticUncertainty-Papers (3)/relatedworks.tex <==
Related Works!

==> problemdef.tex <==
Despite the growing emphasis on accounting for uncertainty in self-adaptive systems~\cite{moreno2016efficient, camara2017reasoning, esfahani2013uncertainty, moreno2018uncertainty}, it has not been addressed at a tactic decision-making process level. Examples of tactic uncertainties, along with motivating examples for them, are described in this section.

% Put into a separate file

% Give some examples of tactic volatility. Perhaps do simulations of leading existing systems to demonstrate that how ?
% Discuss how this could negative impact the system
% >>> Cut down on this from the ASE paper

%\dan{Thurs: Do this}

%Self-adaptive systems typically operate in non-deterministic environments, where the system will encounter numerous unforeseeable events and scenarios. The actions taken by self-adaptive systems will also frequently encounter different forms of volatility, many of which will substantially impact the system's ability to main efficient, and effective. Some forms of volatility include:



% Take much of this from the YIP
\jeff{If we end up running out of room I think the problem definition section could be more concise}
\subsection{Tactic Latency}
The amount of time required to implement a tactic is known as \emph{tactic latency}. Due to various circumstances, these latency times can sometimes become highly volatile. One example tactic could be to access information from a remote server, whose latency time could be volatile due to network or server congestion. As a result, this prevents the system from accurately predicting the behavior of a tactic. Previous works have shown that latency aware algorithms offer several advantages compared to those that do not consider latency~\cite{camara2014stochastic, esfahani2013learning}. However, due to the unpredictable nature of many tactics, their latency times cannot always be accurately estimated. Unfortunately, existing work conducted on decision-making processes in self-adaptive systems also considers tactic latency to be a predetermined, static value. When a system is not able to account for tactic latency volatility or `learn' from previous implementations about what this value may possibly be, this creates uncertainty in the decision making process.  

\subsubsection*{\bfseries Example: Latency Volatility in UAVs}

An unmanned aerial vehicle (UAV), is often used in reconnaissance missions in order to keep soldiers out of harms way. As an example, there may be times when a UAV is flying over an area to locate a certain person with a main goal of taking hi-resolution photos of the area once the person is potentially located. In a scenario where the UAV identities the possible target, several steps must be taken. For this example, we will assume that the UAV needs to physically prepare the camera for taking photos and will need to communicate with the base station while performing other necessary calculations (planned time of .2 seconds). This anticipated latency time means that the UAV should plan on beginning the photography process .2 seconds before it is within range of the possible target. However, in the event of poor weather conditions or something similar, it could take the UAV .4 seconds to communicate with the base station and receive the required data. This would result in the UAV missing its target window for photographing the area, and possibly miss identifying the target entirely. If the UAV was able to use previous knowledge about its prior mission experiences with communication lag, it would enable the UAV to account for tactic latency volatility, further improving the decision-making process for the next time adaptation is required. This example scenario is shown in Figure~\ref{fig:UAVLatencyExampleCamera}. 

\begin{figure*}[ht]
	\centering
    \includegraphics[scale=1.05]{images/UAVCameraExample.PNG}
    \caption{Impact of Unexpected Latency in UAV}
    \label{fig:UAVLatencyExampleCamera}
\end{figure*}




\subsection{Tactic Dependability}
%\subsection{\textbf{Tactic Dependability}} 

In a self-adaptive system certain tactics may be more dependable than others, and having knowledge of this is crucial for the decision-making process. The measure of how well a tactic correctly produces its expected functionality is known as \emph{tactic dependability}. Due to numerous reasons, tactics may sometimes fail to produce their expected results leading to extra consumption of resources or even disastrous consequences in some cases. Therefore, having the ability to estimate when a tactic may or may not work properly is imperative for a self-adaptive system to remain dependable. 
    
\subsubsection*{\bfseries Example: Dependability Volatility in Cloud}

In a cloud-based system, there may be times where interaction with remote computers is required for retrieving necessary information or to make an API call. Due to various reasons, the connection to these remote resources may be inhibited by network congestion or even cyberattacks. Regardless of how well the connections have worked in the past, there will be times where the system attempts to connect to one of the remote computers and gets an unexpected result. For instance, the tactic that connects to a remote computer may only return the expected result 80\% of the time, while the API-call tactic may only return the expected result 90\% of the time. Not being able to account for this in the decision-making process could lead to the system attempting to access the same remote resources every time, even though a similar more dependable resource may be available. 

Figure~\ref{fig:CloudDependabilityExample} displays a possible scenario where a system has three tactic options with identical costs, but with various amounts of produced utility and levels of dependability. If the dependability of each tactic is the same, then selecting the most appropriate tactic is fairly simple; select the one with the highest estimated utility. However, as shown in Figure~\ref{fig:CloudDependabilityExample}, when the dependability and utility of each possible tactic differs, the system must have a way to weigh these differences in order to determine which tactic is most appropriate.

\begin{figure}[h]
	\centering
    \includegraphics[scale=0.85]{images/trade-off.PNG}
    \caption{Impact of Dependability Uncertainty}
    \label{fig:CloudDependabilityExample}
\end{figure}


==> relatedworks.tex <==
Related Works!
